ANOSY: Approximated Knowledge Synthesis with Refinement Types for Declassification

Non-interference is a popular way to enforce confidentiality of sensitive data. However, declassification of sensitive information is often needed in realistic applications but breaks non-interference. We present ANOSY, an approximate knowledge synthesizer for quantitative declassification policies. ANOSY uses refinement types to automatically construct machine checked over- and under-approximations of attacker knowledge for boolean queries on multi-integer secrets. It also provides an AnosyT monad to track the attacker knowledge over multiple declassification queries and checks for violations against user-specified policies in information flow control applications. We implement a prototype of ANOSY and show that it is precise and permissive: up to 14 declassification queries are permitted before a policy violation occurs using the powerset of intervals domain.

==> discussion.tex <==
\section{Discussion}
\label{sec:discussion}

\nv{we need some intro for this section: now it is only clearly addresses the reviews :)}

\paragraph{Security Guarantees}

\tool enforces declassification policies that limit the amount of information an attacker can learn from declassification statements.
%
For this, \tool{} directly checks that downgrades are bounded (\S \ref{sec:monad}) and it relies on the underlying security monad to ensure that the
adversary's knowledge remains constant, \ie there are no leaks, between two @downgrade@s.
%
As a result, the underlying security monad needs to enforce termination-sensitive non-interference.
%
Alternatively, one can use a monad enforcing termination-insensitive non-interference, such as LIO~\cite{stefan2011flexible}, and additionally prove termination, \eg using Liquid Haskell's termination checker.



% \tool's security guarantee holds under the assumption that the
% adversary's knowledge remains constant between two @downgrade@s. We rely
% on the underlying security monad to ensure that no leaks happen between
% downgrades. For example, enforcing non-interference requires use of
% monads like LIO~\cite{stefan2011flexible}, or protecting against
% termination leaks require a termination-sensitive monad.

\mg{Sankha please check my changes to the paragraph above}

\paragraph{Supporting other query classes}
%
\tool can be easily extended to support non-boolean queries with finitely many outputs. 
This can be done 
% In
% practice, any return type that represents a finite set of outputs is
% supported 
by computing one \indset per possible output.
Our technique relies on automatic SMT verification and synthesis, and
it can be extended to other domains with decidable
decision procedures (\eg datatypes). We defer extending \tool with
undecidable secret types (\eg floating points, strings) to future
work.

\paragraph{Policies beyond declassification}

A precise, explicit representation of knowledge as computed by \tool is
at the core of many information flow control tasks. Enforcing
probabilistic policies requires combining knowledge, computed by \tool,
with a probability distribution~\cite{mardziel-beliefpol-2013}. Moreover,
dynamic security policies can be enforced by keeping track of attacker
knowledge and comparing it with the current
policy~\cite{guarnieri2019information}. Finally, approximations of classical
quantitative information flow measures, such as Shannon
entropy~\cite{shannon2001mathematical}, can be derived from the
size of a user's knowledge, \ie the number of concrete elements in the knowledge.


==> encoding.old.tex <==
\section{Refinement Types Encoding}
\label{sec:encoding}

We saw that our bounded downgrade function is correct, 
if each query is coupled with a function @approx@ that correctly 
computes the underapproximation of posterior knowledge. 
Here, we will see how refinement types can specify correctness of @approx@, 
in a way that permite decidable refinement type checking. 


- Abstract Domains 
  - operations (ignore refinements)
  - class laws 
  - type indexes 
%      d:a<p,n> <=> {d: a | \forall x \in d p x \land \forall x \not \in d. n x}
     But foralls inside the refinement preclude decidable verification! 

- Specification of Knowledge 

- Example 1: 
- Example 2: 



In this section we use refinement types to 
encode correct over- and under-approximations 
of the knowledge as defined in~\S~\ref{sec:security}. 
We start with an abstract setting to 
first (\S~\ref{subsec:naive:encoding}) define a general, undecidable encoding
and then (\S~\ref{subsec:decidable:encoding}) 
convert it to decidable one, using abstract refinements. 
Finally, we present two concretizations of our abstract setting: 
the intervals (\S~\ref{subsec:example:intervals})
and powersets (\S~\ref{subsec:example:powersets}) abstract domains.
\sng{to be rewritten}

\begin{figure}
\begin{mcode}
class ADom $\adomtv$ $\cdomtv$ where 
  $\in$ :: $\cdomtv$ -> $\adomtv$ -> Bool
  $\subseteq$ :: $\adomtv$ -> $\adomtv$ -> Bool
  $\cap$ :: d$_1$: $\adomtv$<p$_1$, n$_1$> -> d$_2$: $\adomtv$<p$_1$, n$_1$>
    -> {d$_3$: $\adomtv$<p$_1\land$p$_2$, n$_1\lor$n$_2$> | d$_1 \subseteq$ d$_3$ && d$_2 \subseteq$ d$_3$}
  size      :: $\adomtv$ -> Int
  sizeLaw   :: d$_1$: $\adomtv$ -> {d$_2$: $\adomtv$ | d$_1 \subseteq$ d$_2$}
            -> {size d$_1 \leq$ size d$_2$}
  subsetLaw :: c: $\cdom$ -> d$_1$: $\adomtv$ -> {d$_2$: $\adomtv$ | d$_1 \subseteq$ d$_2$}
            -> {c $\in$ d$_1$ => c $\in$ d$_2$}

$\top$ :: $\adomtv$<{\_ ->  True}, {\_ -> False}>
$\bot$ :: $\adomtv$<{\_ -> False}, {\_ ->  True}>

under_indset::($\adomtv$<{\x ->   query x},{\_ -> True}>,
               $\adomtv$<{\x -> $\lnot$ query x},{\_ -> True}>)
over_indset ::($\adomtv$<{\_ -> True},{\x -> $\lnot$ query x}>,
               $\adomtv$<{\_ -> True},{\x ->   query x}>)

underapprox :: p: $\adomtv$ -> 
  ($\adomtv$<{\x ->   query x $\land$ (x $\in$ p)}, {\_ -> True}>,
   $\adomtv$<{\x -> $\lnot$ query x $\land$ (x $\in$ p)}, {\_ -> True}>)
overapprox  :: p: $\adomtv$ ->
  ($\adomtv$<{\_ -> True}, {\x -> $\lnot$ query x $\lor$ (x $\not \in$ p)}>,
   $\adomtv$<{\_ -> True}, {\x ->   query x $\lor$ (x $\not \in$ p)}>)
\end{mcode}
\caption{Types and definitions \sng{mention that secrets are product of
integer/boolean/float fields?}}
\label{fig:encoding:types}
\end{figure}
  
\subsection{Abstracting Abstract Domains}
\label{subsec:encoding:abstractdom}

Figure~\ref{fig:encoding:types} shows the @ADom@ type class interface to
be implemented by all abstract domains $\adom$. Abstract domains
conceptually represent a set of secrets $\cdom$ given by the definition
of @Concrete $\adom$@. Queries can be any function that accepts a secret
and produces a boolean result. All abstract domains @ADom@ support the
operations:

\begin{enumerate}
  \item Member $\in$: Given a concrete value $\cdom$ and an abstract
  domain $\adom$, it tests if the concrete value is included in the
  abstract domain.
  \item Subset $\subseteq$: Given two abstract domains $\adom$, it tests
  if the first abstract domain is fully included in the second abstract
  domain.
  \item Intersect $\cap$: Given two abstract domains, it computes a new
  abstract domain, that includes all the concrete values that are
  included in both the domains.
  \item Size: Computes the number of concrete values represented by an
  abstract domain.
\end{enumerate}

@subsetLaw@ and @sizeLaw@ as required by @ADom@ does not perform any
computation. These are proof terms, used to verify the semantics of
$\subseteq$ and @size@ are correct. The refinement type on @sizeLaw@
states if @d$_1$@ is a subset of @d$_2$@, then the size of @d$_1$@
should less or equal to @d$_2$@. @subsetLaw@ states, if @d$_1$@ is a
subset of @d$_2$@ then, any concrete value in @d$_1$@ is also in @d$_2$@.

\paragraph{Type-level indexes}

The @ADom@ type class (Figure~\ref{fig:encoding:types}) indexes the
abstract domains with two predicates @p@ and @n@ (@$\cdom$ -> Bool@), or
abstract refinements~\cite{abstract-refinements}.
The positive predicate @p@ describes properties of concrete values that
are members of the abstract domain. Likewise, the negative predicate @n@
describes properties of the values that do not belong to the abstract
domain. This enables the type system to semantically reason about all
values in the domain without quantifiers.
For example, the specification of the full domain @$\top$@
now becomes @$\adom$<{\_ -> True},{\_ -> False}>@, stating that the positive predicate is @True@, \ie satisfied by all elements of the domain, 
and the negative @False@, \ie no elements are outside of the domain.
Similarly, the empty domain @$\bot$@ is now @$\adom$<{\_ -> False},{\_-> True>@, stating the positive predicate is @False@, \ie no elements are
in the domain, and the negative predicate is @True@, \ie all elements
are outside the domain.

The implementations of the abstract domains 
(\eg intervals of~\S~\ref{subsec:encoding:intervals} and powersets
of~\S~\ref{subsec:example:powersets}) 
should be defined so that the elements of the abstraction satisfy @p@ and 
the elements excluded @n@. There is no requirement that these two
predicates are complementary or even mutually exclusive. 
For example, if @IntAbs@ is an abstraction over integers (\ie represents
a set of integers), then the three alternatives below describe abstractions 
that include only natural numbers (\ie the positive predicate @p@ instantiated 
to @\x -> 0 <= x@).
\begin{mcode}
precise   :: IntAbs <{\x -> 0 <= x},{\x -> x < 0}>
imprecise :: IntAbs <{\x -> 0 <= x},{\_ ->  True}>
bounded   :: IntAbs <{\x -> 0 <= x},{\x -> x < 4}>
\end{mcode}
In @precise@, the negative predicate @\x -> x < 0@ is a complement of the positive, precisely describing the abstraction to be the natural numbers. 
In @imprecise@ the negative predicate is true, capturing no information 
for the elements that do not belong in the abstraction, 
thus the abstraction can be \textit{any} subset of the natural numbers. 
Finally, in @bounded@ the negative predicate @\x -> x < 4@ intersects the positive, leaving only unspecified if the elements of the intersection [0,3] belong or not in the abstract domain. 
% \nv{Checked this...}
% http://goto.ucsd.edu:8090/index.html#?demo=permalink%2F1620307140_33798.hs
In summary, as is usual for refinement type specifications, 
the index predicates do not enforce completeness in the abstraction description.
% They instead ensure that all the elements in (\resp outside of) the domain 
% satisfy the positive (\resp negative) predicate. 
% The more precise the predicate, the more information it gives for the domain, 
% but as usual in refinement type specifications, the more difficult 
% type checking becomes. 

Next, we use these type indices to verify the intersection semantics of
abstract domains.

\paragraph{Intersection of Abstract Domains}

In general, the intersection of two abstract domains cannot be precisely
represented in the same abstract domain. For example, the set of values
represented by the intersection of two octagons
(Figure~\ref{fig:posterior:knowledge}) is not precisely captured by an
octagon, but can be approximated by 
an octagon. Thus, a valid intersection is any octagon that is a subset
of the precise intersection. However, doing this requires tracking all
values in each of the abstract domains, which is aided by our type-level
indexes. Hence, the type signature for intersect $\cap$ returns a
domain @d$_3$@ whose positive predicate indicates it includes elements
included in @d$_1$@ and @d$_2$@ \ie @p$_1 \land$p$_2$@. The negative
predicate indicates points excluded from @d$_3$@ are points excluded
from either @d$_1$@ or @d$_2$@, \ie @n$_1 \lor$n$_2$@. The refinement on
@d$_3$@ ensure that @d$_3$@ is a subset $\subseteq$ of both @d$_1$@ and
@d$_2$@.

% The specification of the intersection type (shown in
% Figure~\ref{fig:code:decidable}), 
% % exactly 
% captures the propagation of the two indexes: 
% the positive predicate is the conjunction and the negative a disjunction 
% of the respective argument predicates.
% This precise specification exactly propagates the information of 
% the indexed predicates and 
% allows 
% % the 
% clients of the conjunction 
% to get verified. 
% yet verification of the implementation of $\cap$ itself is a challenging process
% (as discussed in the two concrete abstractions below \S~\ref{subsec:example:intervals} and~\ref{subsec:example:powersets}).  
% SILENT THIS :)
% \nv{Sankha check above and what happened with the intersection
% proofs?}

\subsection{Approximations}
\label{subsec:encoding:approxes}

\paragraph{Approximations of \indsets}

The specification of the under-approximation of the \indset @under_indset@
says the first domain only includes secrets for which the @query@ is
@True@, and the second domain only includes secrets for which the
@query@ is @False@ (the positive predicate). The negative predicates do
not impose any constraints on the elements that do not belong to the
domain. This means the domains can exclude any number of secrets, as
long as the secrets that are included are correct, \ie it is an
under-approximation.

Dually, the over-approximation @over_indset@ sets the negative predicate to
exclude all points for which the @query@ evaluates to @False@ for the
domain corresponding to @True@ response, and the second domain
(corresponding to response @False@) excludes all points that evaluate to
@False@ with @query@. The over-approximate \indsets do not put any
restrictions on the points that have to be included in the domain. Here
the domains can include any number of secrets as long as they are not
leaving out any secrets that are correct, \ie it is an
over-approximation.

\paragraph{Approximations of knowledge}

The \indset approximations are query specific and they approximate the
set of inputs that result in different result from the query. However,
an attacker might already have some knowledge about the secret, either
from observing results of previous queries or by having a large enough
set of assumptions to cover all possible secrets. By combining the prior
knowledge of the attacker with the \indset for the query, we can derive
an approximation of the attacker's knowledge if they observe the query.

Figure~\ref{fig:encoding:types} shows the specification for the
knowledge under-approximation @underapprox@, and the over-approximation
@overapprox@. @underapprox@ is similar to the type of @under_indset@,
except the positive predicate is strengthened to express that  
all the elements of the domain should also belong to the prior knowledge
@p@. Similarly, @overapprox@ specifies that the elements that do not
belong in the posterior knowledge, should neither be in the prior nor
the \indset.

\paragraph{Precision}

The refinement types ensure our definitions are correct, 
but they do not reason about the precision of the derived abstract domains. 
For example, the bottom $\bot$ and top $\top$ domains 
are vacuously correct solutions for under- and over-approximations, 
respectively. But, these domains are of no use, since they ignore all
the query information. In general a domain is more precise for an
under-approximation if its size is higher, and conversely, an
over-approximation is more precise if its size is lower.

Next, we present some concrete instances of our abstract domains:
intervals (\S~\ref{subsec:encoding:intervals}), powersets of intervals
(\S~\ref{subsec:encoding:powersets}).

\subsection{Interval Domain}
\label{subsec:encoding:intervals}

Next we define \adomi, the interval abstract domain 
that can be used as an abstraction for any secret type, constructed from
fields with integer types (like the @UserLoc@ secret type
of~\S~\ref{sec:overview}). In practice, secrets being expressed as
product type of integers has not been limiting, as we can express
different types like booleans, enums, etc as integers. \adomi is defined
as below:

\begin{mcode}
data Interval = Interval {
  lower :: Int
, upper :: {v:Int | lower <= v }}

type Proof p x = {v:$\cdom$<p> | v = x }

data $\adomi$ <p::$\cdom$ -> Bool, n::$\cdom$ -> Bool> 
  = $\adomi$ { dom :: [Interval]
        , pos :: x:{$\cdom$| x $\in$ dom } -> Proof p x  
        , neg :: x:{$\cdom$| x $\not \in$ dom } -> Proof n x }
  | $\topi$ { pos :: x:$\cdom$ -> Proof p x }
  | $\boti$ { neg :: x:$\cdom$ -> Proof n x }
\end{mcode}

$\adomi$ has three constructors. $\topi$ and $\boti$ respectively denote
the complete and empty domains. @$\adomi$@ represents the domain of any
n-dimensional intervals, where @n@ is the length of @dom@. Intervals
represent integers between @upper@ and @lower@. For a secret
$\concval = \concval_1 \times \concval_2 \times \ldots \concval_n$,
\sng{show this product type in \S~\ref{subsec:encoding:abstractdom}?} the
abstract domain \adomi represents all secrets
@$\concval_1 \in$ (dom!1), $\ldots$, $\concval_i \in$ (dom!i), $\ldots$, $\concval_n \in$ (dom!n)@
in the @n@ dimensional space. For example, 
@dom = [(Interval 188 212), (Interval 112 288)]@  
is the rectangle of $x \in [188, 212], y \in [112, 288]$ in the two
dimensional space of @UserLoc@.
% This encoding, where @dom@ is a list, let us abstract over 
% secret types that contain \textit{any} number of integer components, 
% since lists can have \textit{any} number of elements, 
% one for each integer component. 

\paragraph{Proof Terms}
The @pos@ and @neg@ components in the $\adomi$ definition 
are proof terms that give meaning to the positive @p@ and negative @n@
abstract refinements.
The complete domain \topi contains the proof field @pos@
that states that every secret \concval\ should satisfy the 
positive predicate @p@ (\ie @x: $\cdom$ -> Proof p x@), and the empty
domain contains only the proof @neg@ for the negative predicate @n@.
Due to syntactic restrictions that abstract refinements can only be
attached to a type for SMT-decidable
verification~\cite{abstract-refinements}, the proof terms terms are
encoded as functions that return the secret, while providing evidence
that the respective predicates is inhabited by possible secrets.
In \adomi this is encoded by setting preconditions to the
proof terms: the type of the @pos@ field states that each @s@ that
belongs to @dom@ should satisfy @p@, while the @neg@ field states that
each @x@ that does not belong to @dom@ should satisfy @n@ (see
\S~\ref{sec:overview} for an example \sng{put an example in
\S~\ref{sec:overview}}).

% The encoding of these proof terms is complicated 
% because of the strict syntactic restriction
% (required for SMT-decidable checking) that abstract refinements 
% can only be attached to a type.  
% Thus instead of ideally encoding proof terms as unit values 
% refined to show @p x@, we equivalently show that 
% each @x@ can be refined with the abstract refinement @p@: 
% \begin{mcode}
% pos :: x:s -> {v:()   | p x  } -- ideal proof encoding 
% pos :: x:s -> {v:s<p> | v = x} -- equivalent encoding
% \end{mcode}
% We use the type alias @type Proof s p x = {v:s<p> | v = x }@ to hide % away 
% this complicated proof encoding, 
% but the evidence % (or inhabitants) 
% of such proof terms are still required to be expressions 
% of type @s@. For example, the following shows that each element @x@ proves the true predicate. 
% \begin{mcode}
% propTrue :: x:s -> Proof s {\_ -> True} x 
% propTrue x = x
% \end{mcode}

% Dually to top, the bottom constructor, carries a proof 
% that each element of @s@ satisfies the negative predicate @n@, 
% setting up the meaning of the index refinements: 
% @p@ is satisfied by each element in the domain and @n@ by each element 
% outside of the domain. 


% \paragraph{The Ship Example}
% \begin{figure}
% \begin{mcode}
% -- User Specified Input (as in $\S~\ref{sec:overview}$)
% data Ship = Ship { x :: Int, y :: Int} 
% nearby :: Ship -> Bool
% nearby s = abs (x s - 200) + abs (y s - 200) <= 100
% \end{mcode}
  
% \begin{mcode}
% -- $\tool$ Synthesized Output
% $\in$ :: Ship -> $\adomi$ Ship -> Bool 

% under_indset :: s:Ship -> 
%   $\adomi$ Ship<{\x -> nearby s <=> nearby x}, {\_ -> True}>
% over_indset  :: s:Ship -> 
%   $\adomi$ Ship<{\_ -> True}, {\x -> not (nearby s <=> nearby x)}>  

% under_post :: s:Ship -> p:$\adomi$ Ship ->
%   $\adomi$ Ship<{\x$\,$->$\,$(nearby s <=> nearby x)$\,$$\land$$\,$(x$\in$p)},{\_$\,$->$\,$True}>
% under_post s p = refine p $\cap$ under_indset s 
% over_post  :: s:Ship -> p:$\adomi$ Ship ->
%   $\adomi$ Ship<{\_$\,$->$\,$True},{\x$\,$->$\,\lnot\,$(nearby s$\,$<=>$\,$nearby x)$\,\lor\,$(x$\not\in$p)}>  
% over_post s p = refine p $\cap$ over_indset s 

% refine$\,$::$\,$x:$\adomi$ s$\,$->$\,${r:$\adomi$ s<{\v$\,$->$\,$v$\in$x},{\v$\,$->$\,$$\lnot$(v$\in$x)}>$\,$|$\,$v = x}
% refine x = x 
% \end{mcode}
% 
% \caption{\small The Ship Example as Synthesized by $\tool$.}
% \label{fig:code:ship:decidable}
% 
% \end{figure}
% Figure~\ref{fig:code:ship:decidable} summarizes how the $\adomi$ abstract domain 
% instantiates the encoding of Figure~\ref{fig:code:decidable} 
% to synthesize the over- and under-approximations of the Ship example from~\S~\ref{sec:overview}.
% %
% We have defined the Interval Domain Library 
% that includes the indexed data type $\adomi$ and 
% the top domain (@$\top$@) that is simply the top constructor 
% with the true proof term. 
% Our library further includes the subset and union verified operators 
% that can be found in our implementation. 
% As presented in~\S~\ref{sec:overview}, the user 
% specifies the secret data type to be the @Ship@ 
% (in general, any non-recursive data type with integer only components)
% and @nearby@ to be a boolean query on the secret type. 
% Finally, $\tool$ will mechanically (\ie using syntax directed boilerplate code) 
% synthesize the $\in$ operator and the specifications for the over- and under-approximations 
% for the \indsets and posterior knowledge. 
% The implementation of the posterior knowledges is also mechanically produced,
% as the conjunction of the (properly refined) posterior with the respective 
% \indset. 
% The implementation of the \indsets is challenging as it requires 
% solving tedious constraints and is discussed in details in~\S~\ref{sec:synthesis}. 
% Here, for completeness of this example, we present the synthesized code for 
% the @under_indset@ function: 
% \begin{mcode}
%   under_indset :: s:Ship -> 
%      $\adomi$ Ship <{\x -> nearby s <=> nearby x},{\_ -> True}> 
%   under_indset s = case (nearby s)  of
%     True  -> $\adomi$ [Interval 121 279, Interval 179 221]  
%                  propTruePos  propTrue
%     False -> $\adomi$ [Interval 0 400, Interval 0 99]  
%                  propFalsePos propTrue

%   propTruePos :: s:{Ship | 121$\;$<=$\;$x s$\;$<=$\;$279$\;$&&$\;$179$\;$<=$\;$y s$\;$<=$\;$221}
%               -> Proof Ship {\v -> nearby v} s
%   propTruePos s = s

%   propFalsePos :: s:{Ship | 0 <= x s <= 400 && 0 <= y s <= 99}
%                -> Proof Ship {\v -> $\lnot$ (nearby v)} s
%   propFalsePos s = s
% \end{mcode}
% %
% The definition of @under_indset@ case splits on the result of the query 
% and in each case it returns a two dimensional rectangle that matches the query 
% together with explicit proof terms. 
% \tool will synthesize the above tedious code with the required explicit proofs 
% and will further use Liquid Haskell 
% to automatically verify that the code indeed satisfies the @under_indset@, under-approximation 
% specification. 

\paragraph{Implementation}

The \adomi domain is backed by interval arithmetic lifted to
n-dimensions. $\in$ checks if any secret is between @lower@ and
@upper@ for every dimension. $\subseteq$ checks if the intervals
representing the first argument is included in the intervals
representing the second argument. $\cap$ computes a new list of
intervals to represent the abstract domain, that includes only the
common concrete values of the arguments. We skip the definitions for
empty and full domains due to space, but they behave like standard
abstract domains. Size just computes the number of secrets in the
domain, which can be interpreted as the volume.

\begin{mcode}
$\in$ :: $\cdom$ -> $\adomi$ -> Bool
$\in$ ($\concval_1 \times \ldots \times \concval_n$) (Range b _ _) = $\bigwedge\limits_{i}$ inInd $\concval_i$ b!i
  where inInd i (Interval l u) = l $\leq$ i $\land$ i $\leq$ u

$\subseteq$ :: $\adomi$ -> $\adomi$ -> Bool
$\subseteq$ (Range b$_1$ _ _) (Range b$_2$ _ _) = $\bigwedge\limits_{i}$ ssInd b$_1$!i b$_2$!i
  where ssInd (Interval l$_1$ u$_1$) (Interval l$_2$ u$_2$) = l$_2$ $\leq$ l$_1$ $\land$ u$_1$ $\leq$ u$_2$

$\cap$ :: $\adomi$ -> $\adomi$ -> $\adomi$
$\cap$ (Range b$_1$ p$_1$ n$_1$) (Range b$_2$ p$_2$ n$_2$) =
  if $\bigwedge\limits_{i}$ validInd b$_1$!i b$_2$!i then
    Range [$\ldots$, (interInd b$_1$!i b$_2$!i), $\ldots$] (intersectP p$_1$ p$_2$) (intersectN n$_1$ n$_2$)
  else $\boti$ where
validInd (Interval l$_1$ u$_1$) (Interval l$_2$ u$_2$) = l$_2 \leq$ u$_1 \lor$ l$_1 \leq$ u$_2$
interInd (Interval l$_1$ u$_1$) (Interval l$_2$ u$_2$) = Interval (max l$_1$ l$_2$) (min u$_1$ u$_2$)

size :: $\adom$ -> Int
size (Range b _ _) = (sizeInd b!1) * $\ldots$ * (sizeInd b!n)
  where sizeInd (Interval l u) = u - l + 1
\end{mcode}

As our implementation is backed by lists to support
secrets with arbitrary number of fields, LiquidHaskell fails to prove
@subsetLaw@ and @sizeLaw@ automatically.
However, we proceed by providing the induction step to
LiquidHaskell and the individual cases are proved automatically. Below,
we show how the proof proceeds, by simplifying the representation from
our data type to lists. Our implementation performs the proofs over the
types described above. @subsetIntLaw@ shows that property holds for each
individual interval, and then @subsetLaw@ combines this with the
recursive step to prove that the property holds for n-dimensional
intervals. Our encoding as lists necessitates additional preconditions
the number of fields in the secret is the same the number of intervals
in the abstract domain.

\begin{mcode}
{-@ subsetIntLaw :: i: Int -> r1: Interval
  -> {r2: Interval | r1 $\subseteq$ r2}
  -> {i $\in$ r1 => i $\in$ r2} @-}
subsetIntLaw :: Int -> Interval -> Interval -> ()
subsetIntLaw i r1 r2 = ()

{-@ subsetLaw :: i: [Int] -> r1: [Interval]
  -> {r2: [Interval] | (r1 $\subseteq$ r2)
          && (len i == len r1) && (len i == len r2)}
  -> {i $\in$ r1 => i $\in$ r2} @-}
subsetLaw :: [Int] -> [Interval] -> [Interval] -> ()
subsetLaw [] [] [] = ()
subsetLaw (x:xs) (y:ys) (z:zs) = (subsetIntLaw x y z) ? subsetLaw xs ys zs
\end{mcode}

% \paragraph{Abstract Refinements}
% Abstract refinements~\cite{abstract-refinements}
% allow indexing data types with abstract predicates. 
% As a trivial example the data definition @IntUnit@ below 
% is indexed with the predicate @p@ on integers 
% that should be satisfied by its integer component (@intc@). 
% \begin{mcode}
%   data IntUnit <p :: Int -> Bool> = 
%        IntUnit {intc :: Int<p>, unitc :: ()}
% \end{mcode}
% %
% The meaning of the indexes is given by the definition of the data types. 
% In the @IntUnit@ definition, the @intc@ has type @Int<p>@ which is
% Liquid Haskell's syntax for @{v:Int | p v}@. 
% Thus, the integer component of @IntUnit<p>@ should satisfy @p@. 
% For example, when the integer component is @42@, the predicate 
% can describe positive, but not negative numbers: 
% \begin{mcode}
%   IntUnit 42 () :: IntUnit <{\v -> 0 < v}> -- ok
%   IntUnit 42 () :: IntUnit <{\v -> v < 0}> -- error
% \end{mcode}

% Data can be parameterized with multiple abstract refinements. 
% For example, the @IntInt@ data type below has two abstract refinements, 
% one for each of its integer components. 
% \begin{mcode}
%   data IntInt <p1 :: Int -> Bool, p2 :: Int -> Bool> 
%     = IntInt {int1 :: Int<p1>, int2 :: Int<p2>}
% \end{mcode}
% %
% With the above definition, in @IntInt<p1, p2>@, @p1@
% describes the first integer components and @p2@ the second. 
% For example, below we describe an @IntInt@ 
% that has a positive 
% first component and a negative second component. 
% %
% \begin{mcode}
%   IntUnit 4 -4 :: IntUnit <{\v -> 0$\,$<$\,$v},{\v -> v$\,$<$\,$0}> -- ok
% \end{mcode}
% \citet{abstract-refinements} describe how abstract refinements are encoded 
% using uninterpreted functions to allow decidable type checking. 
% Here we make use of this technology to 
% define abstract domains indexed with properties of their concrete elements. 

\subsection{Powersets of Intervals}
\label{subsec:encoding:powersets}

To address the imprecision of the interval abstract domains, 
we follow the technique of~\cite{powerset1,powerset2} and define 
the powerset abstract domain \adomp \ie a set of interval domains. 
Similar to intervals (\S~\ref{subsec:encoding:intervals}), powerset
\adomp is also parameterized with the positive and negative predicates:
%
\begin{mcode}
data $\adomp$ <p::$\cdom$ -> Bool, n::$\cdom$ -> Bool> = $\adomp$ {
    dom_i :: [$\adomi$]
  , dom_o :: [$\adomi$]
  , pos :: x:{$\cdom$|x $\in$ dom_i $\land$ x $\not\in$ dom_o} -> Proof p x  
  , neg :: x:{$\cdom$|x $\not\in$ dom_i $\lor$ x $\in$ dom_o} -> Proof n x}
\end{mcode}
%
\adomp contains four fields. 
@dom_i@ is the set (represented as a list) of intervals
that are contained \emph{in} the powerset.
@dom_o@ is the set of intervals that are \emph{excluded} from the
powerset. This representation backed by two lists gives flexibility to
define powersets by writing regions that should be included and
excluded, without sacrificing generality or correctness (as guaranteed
by our proofs). Moreover, this encoding of the powerset makes our
synthesis algorithm simpler (\S~\ref{sec:synthesis}).
% To precisely represent domains -- especially over-$\!$ approximations,
% as we shall see next --  
% it is ofter convenient to \textit{exclude} intervals from the
% abstraction. 
The proof terms provide the boolean predicates that give semantics to
the secrets contained in the powerset, as similar to the interval domain
(\S~\ref{subsec:encoding:intervals}). We do not need a separate top
$\top$ and bottom $\bot$ for \adomp as they can be represented using
\topi or \boti in the @pos@ list.

\paragraph{Implementation}

A concrete value belongs to ($\in$) the powerset \adomp if it belongs
to any individual interval of the @dom_i@ list but not in any individual
interval of the @dom_o@ list. The subset ($\subseteq$) operation checks
if all the individual intervals in the inclusion list @dom_i@$_1$ is a
subset of atleast one interval in the inclusion list @dom_i@$_2$, and
also that none of the individual intervals in the exclusion list
@dom_o@$_1$ is a subset of any interval in @dom_o@$_2$. This operation
returns @True@ is the the first powerset is a subset of the second, but
if it returns @False@ it may or may not be powerset. We have not found
this to be limiting in practice, as this criteria is sufficient for
verification. We plan to improve the accuracy via better algorithms
\sng{cite?} in future work. Intersection $\cap$ produces a new powerset,
whose inclusion list is made of pair-wise intersecting intervals from
@dom_i@$_1$ and @dom_i@$_2$, and the exclusion interval list is simply the
union of all intervals in the individual exclusion lists @dom_o@$_1$, and
@dom_o@$_2$. Size is computed by taking the sum of size of all intervals
in the inclusion list less the size of size of all intervals in the
exclusion list.

\begin{mcode}
$\in$ :: $\cdom$ -> $\adomp$ -> Bool
$\in \concval$ ($\adomp$ dom_i dom_o _ _) = ($\bigvee\limits_{i}$ $\concval \in$ dom_i!i) $\land$
  ($\lnot \bigvee\limits_{i}$ $\concval \in$ dom_o!i)

$\subseteq$ :: $\adomp$ -> $\adomp$ -> Bool
$\subseteq$ ($\adomp$ dom_i$_1$ dom_o$_1$ _ _) ($\adomp$ dom_i$_2$ dom_o$_2$ _ _) =
  ($\bigwedge\limits_{i,j}$ dom_i$_1$!i $\subseteq$ dom_i$_2$!j) $\land$ ($\bigwedge\limits_{i,j}$ dom_o$_2$!i $\subseteq$ dom_o$_1$!j)

$\cap$ :: $\adomp$ -> $\adomp$ -> $\adomp$
$\cap$ ($\adomp$ dom_i$_1$ dom_o$_1$ p$_1$ n$_1$)($\adomp$ dom_i$_2$ dom_o$_2$ p$_2$ n$_2$) =
  $\adomp$ [$\ldots$, (dom_i$_1$!i $\cap$ dom_i$_2$!j), $\ldots$] (dom_o$_1$ ++ dom_o$_2$) (intersectP p$_1$ p$_2$) (intersectN n$_1$ n$_2$)

size :: $\adomp$ -> Int
size ($\adomp$ dom_i dom_o _ _) = (size dom_i!1) + $\ldots$
  + (size dom_i!n) - (size dom_o!1) - $\ldots$ - (size dom_o!n)
\end{mcode}

We omit the proofs for @subsetLaw@ and @sizeLaw@ as the proofs proceed
similar to the interval domain (\S~\ref{subsec:encoding:intervals}) by
manually providing the induction step. \sng{show an example of powerset?}

% subset = True indicates it is a subset, subset = False means it
% may/may not be a subset

% \paragraph{The Ships Example.}
% \begin{figure*}
% \centering
% \begin{subfigure}[b]{0.3\textwidth}
% \includegraphics[width=\textwidth]{ship-under-power}

% \caption{\small  Under-Approximation}
% \label{fig:nearby:under:pow}
% \end{subfigure}%
% \begin{subfigure}[b]{0.7\textwidth}
% \begin{mcode}
%   under_indset :: s:Ship -> $\adomp$ Ship<{\l -> nearby secret <=> nearby l},{\_ -> True}> 
%   under_indset s = case (nearby s) of 
%     True -> ($\adomp$ [
%             ($\adomi$ [(Interval 121 279), (Interval 179 221)] _ _) -- t:1
%           , ($\adomi$ [(Interval 145 255), (Interval 222 245)] _ _) -- t:2
%           , ($\adomi$ [(Interval 149 251), (Interval 151 178)] _ _) -- t:3 
%           ] [] _ _)
%     False -> ($\adomp$ [
%             ($\adomi$ [(Interval   0 400), (Interval   0  99)] _ _) -- f:1
%           , ($\adomi$ [(Interval   0  99), (Interval 100 400)] _ _) -- f:2 
%           , ($\adomi$ [(Interval 301 400), (Interval 100 400)] _ _) -- f:3
%           ] [] _ _)
% \end{mcode}

% \caption{\small Powerset Under-Approximation Posterior Definition}
% \label{fig:nearby:under:pow:code}
% \end{subfigure}
% \begin{subfigure}[b]{0.3\textwidth}
% \includegraphics[width=\textwidth]{ship-over-power}

% \caption{\small Over Approximation}
% \label{fig:nearby:over:pow}
% \end{subfigure}%
% \begin{subfigure}[b]{0.7\textwidth}
% \begin{mcode}
%   over_indset :: s:Ship -> $\adomp$ Ship<{l:Ship | },{\_ -> not (nearby secret <=> nearby l)}> 
%   over_indset s = case (nearby s) of 
%     True -> ($\adomp$ [
%             ($\adomi$ [(Interval 100 300), (Interval 100 300)] _ _) -- t:1
%           ][
%             ($\adomi$ [(Interval 226 300), (Interval 100 125)] _ _) -- t:2
%             ($\adomi$ [(Interval 219 300), (Interval 282 300)] _ _) -- t:3
%           ] _ _)
%     False -> ($\adomp$ [
%             ($\adomi$ [(Interval   0 400), (Interval   0 400)] _ _) -- f:1
%           ] [] _ _)
% \end{mcode}

% \caption{\small Powerset Over-Approximation Posterior Definition}
% \label{fig:nearby:over:pow:code}
% \end{subfigure}
% \caption{\small Indistinguishability Sets for the ship example using the powerset abstract domain.}
% \label{fig:nearby-example-pow}

% \end{figure*}
% Figure~\ref{fig:nearby-example-pow} presents the \indsets of 
% our running ship example, using powersets. 
% Now the under-approximation (\ref{fig:nearby:under:pow})
% consists of three rectangles for both the true (t:1-3)
% and the false (f:1-3) case. At both cases the interval abstraction 
% contains only the first of the three rectangles, thus is clearly less precise. 
% %Over-approximations cannot be precisely abstracted as a union of abstractions, 
% %since to gain precision areas need to be excluded.
% %
% \ref{fig:nearby:over:pow} presents the over-approximation, where 
% in the true case, the rectangles t:2 and t:3 are excluded to gain precision. 
% The false case remains the same as in the interval abstraction, containing 
% all the domain. At the right of figure~\ref{fig:nearby-example-pow} we present 
% the definitions of the \indsets with the proof terms replaced with wildcards.
% It is clear that the generation of such definitions is a tedious and error prone process, 
% thus next we describe how they are automatically synthesized by \tool. 


==> monad.old.tex <==
\section{\tool Monad}
\label{sec:monad}

\begin{figure}
\begin{center}
  \includegraphics[width=0.3\textwidth]{knowledge_venn}
\end{center}
\caption{\small The knowledge ($K$) is the intersection of prior
knowledge ($P$) with the \indset on $q$ for the secret $s$ ($q\ x = q\
s$). \sng{replace with octagon and new notation}}
\label{fig:posterior:knowledge}
\end{figure}

\paragraph{Tracking knowledge of secrets}

We consider an attacker who can learn information about the secret
\cdom, by observing the results of executing the @query@. To protect
against information leakage, the system
needs to quantify the attacker's knowledge of the set secrets they
consider possible. As the adversary runs more queries, they learn more
information about the secret, and their knowledge (or the set of
possible secrets) evolves along with it.

A @query@ partitions the set of secrets \cdom into two indistinguishable
set of secrets
$\cdom_t$ and $\cdom_f$, for the true and false boolean results respectively.
In other words, all secret values $s \in \cdom_t$ that produce the
output @True@ in response to @query@, \ie $\cdom_t = \{ s\in \cdom_t
\mid \texttt{query}\ s \}$. Similarly, all secrets in $\cdom_f$
evaluates to @False@ in response to query, \ie $\cdom_f = \{ s\in \cdom_f
\mid \lnot\ \texttt{query}\ s \}$.
% \footnote{$I_{q,\texttt{tt}}$ and
% $I_{q,\texttt{ff}}$ are the two equivalence classes induced by the
% indistinguishability equivalence relation $\sim_q$ such that $s \sim_q
% s'$ iff $q\ s = q\ s'$~\cite{backesleak09}.}
Hence, attackers (without further information) that observe the output
as @True@ or @False@, only know that the secret is one of the values in
$\cdom_t$ or $\cdom_f$ respectively, but they cannot obtain any further
information. We refer to the set of secrets inferred from the output as
$\cdom_O$ for brevity, it is always $\cdom_t$ or $\cdom_f$ depending on
the output.

An attacker, that starts off with an initial assumption for the set of
secrets $\cdom_P$ (called the \emph{prior}), updates their knowledge as
they observe outputs of the queries. This updated knowledge (also called
the \emph{posterior}) can be derived by including only the set of
secrets from the prior that are consistent with the observed result from
the query \ie $\cdom_P \cap \cdom_O$; see
Figure~\ref{fig:posterior:knowledge} for a 
graphical representation. The knowledge learned from a sequence of $n$
such queries can be generalized to $\cdom_P \cap \cdom_{O,1} \cap
\cdom_{O,2} \ldots \cap \cdom_{O,n}$, where $\cdom_{O,i}$ is the
indistinguishable set of $i$-th query.

\paragraph{Approximating knowledge}

Operations over such a set of secrets requires us to reason about all
secrets (corresponds to the forall $\forall$ quantifier in logic), an
undecidable task in general. Hence, a more tractable way is to
approximate the set of secrets as abstract domains \adom, on which we
can define operations efficiently. We present the detailed descriptions
of such abstract domains in \S~\ref{sec:encoding}.
Any secret represented in an
under-approximate \indset $\absval_u: \adom$ for a query,
is always included in the precise \indset, \ie @s $\in
\absval_u \Rightarrow$ s $\in \cdom_O$@. Conversely, an over-approximate
\indset $\absval_o: \adom$ for a query has all secrets represented by
the precise \indset, \ie @s $\in \cdom_O \Rightarrow$ s $\in
\absval_o$@. Consequently, the under-approximate, and the over-approximate
posterior knowledge can be computed by taking the intersection of the
prior with the corresponding approximate \indset. Together, the under-
and over-approximate posteriors form a lower and upper bound on the
amount information an attacker can have about the secret.

\begin{figure}
\begin{mcode}
query :: $\cdom$ -> Bool

type AnosyT $\adom$ $\cdom$ m = StateT ({
  prior  :: $\adom$
, policy :: $\adom$ -> Bool
, secret :: Maybe $\cdom$}) m

downgrade :: Monad m
          => query :  ($\cdom$ -> Bool)
          -> approx: ($\adom$ -> ($\adom$, $\adom$))
          -> AnosyT $\adom$ $\cdom$ m Bool
downgrade query approx = do
  st <- get
  let (postT, postF) = approx (prior st)
  if (policy postT) && (policy postF)
      && isJust (secret st) then do
    let response = query (fromJust (*\$*) secret st)
    let newPrior = if response then postT else postF
    modify (*\$*) \st -> st { prior = newPrior }
    return (*\$*) response
  else return (*\$*) throw (*\$*) userError "unsafe"
\end{mcode}
\caption{The \texttt{AnosyT} monad transformer and definition of
\texttt{downgrade}}
\label{fig:monad-downgrade}
\end{figure}

\paragraph{Enforcing policies for declassification}

Whenever an adversary learns some information about the secret, it is a
declassification. \sng{mention non-interference?} Given enough chances
to run the query, the adversary can guess the secret exactly. To limit
the information an adversary learns from the execution of queries, a
programmer can put in place a security policy @ADom -> Bool@, a function
that can test if an approximation of the knowledge satisfies some
criteria to ensure the the adversary cannot precisely guess the secret.
In practice, it often tests if the number of secrets represented by the
abstract domain are more or less than some bound.

Figure~\ref{fig:monad-downgrade} shows the @AnosyT@ monad, a state
transformer, which wraps any user computation, while carrying the 
information about the prior, policy and secret. These three are used to
safely declassify the secret using 
the @downgrade@ function. The downgrade function given a @query@, and a
corresponding approximation function @approx@, that estimates the posterior
knowledge for both @True@ and @False@ response, safely declassifies the
result of computation of a query. The @downgrade@ function evaluates to
the response of the query if all 
possible posteriors conform to the policy, while updating the monad
state to use the relevant posterior as the new prior. This ensures the
same monad can be used for safe declassification of the result of
multiple queries.


==> overview.old.tex <==
\section{Overview}
\label{sec:overview}

\subsection{Setup}
% \todo{Marco does this}
% \todo{define what is means for a function to be sound}


% \mg{How do we plan to structure overview? (1) discuss example setup (ships, points, ...)
% (2) discuss security concerns (3) discuss soundness and complementess}

\begin{figure}
  \begin{subfigure}[]{0.49\textwidth}
    \begin{mcode}
data Ship = Ship {
  capacity :: Int,
  x        :: Int,
  y        :: Int
}

{-@ reflect abs @-}
abs :: Int -> Int
abs i | i < 0 = -1 * i
abs i         = i

{-@ reflect nearby @-}
nearby :: Ship -> Bool
nearby secret = (capacity secret) > limit && (abs (x secret - 200) + abs (y secret - 200) <= d)
  where
    limit = 50
    d = 100

{-# ANN Ship ([
  ("capacity", (0, 100)),
  ("x", (0, 500)),
  ("y", (0, 500))
  ] :: [(String, (Int, Int))]) #-}

{-# ANN module ("sound", "nearby") #-}
{-# ANN module ("complete", "nearby") #-}\end{mcode}
    \caption{Ships problem spec}
    \label{fig:ship-spec}
  \end{subfigure}
  \hfill
  \begin{subfigure}[]{0.49\textwidth}
    \begin{mcode}
data IntRange = IntRange { lower :: Int, upper :: Int}

data LocRange <p :: Loc -> Bool, n :: Loc -> Bool> = LocRange {
  xr :: IntRange
, yr :: IntRange }

{-@ sound :: secret:Loc
-> {prior:LocRange | secret $\in$ prior}
-> {post:LocRange<{p:Loc | nearby secret <=> nearby p},{\_->True}|post $\subseteq$ prior> 
@-}
sound secret prior@(LocRange (IntRange xl xu) (IntRange yl yu)) =
case (nearby secret) of
True  -> LocRange
    (IntRange (max xl 188) (min xu 212))
    (IntRange (max yl 112) (min yu 288))
False -> LocRange
    (IntRange (max xl 301) (min xu 500))
    (IntRange (max yl   0) (min yu 500))\end{mcode}
    \caption{manually written solution}
    \label{fig:ship-soln-manual}
  \end{subfigure}
  \caption{Ships problem}
\end{figure}


Consider a \emph{ship} that wants to allow any third party (including
potential \emph{adversaries}) to execute arbitrary computations over her
location. Figure~\ref{fig:ship-spec} shows a sample implementation of
the problem, simplified from one of our benchmarks


For this, the ship accepts programs written by the adversary,
executes them locally, and returns their results back. The ship,
however, is concerned about what an adversary could learn about the
ship's precise location from these results. Hence, the ship
models the prior knowledge the adversary might have, and then estimates
the potential information leakage by running the computation and then
choose to not run it if answering the query might lead to a security
policy violation.

% \mg{We need to stress more the idea that knowledge is the set of all possible secret values}

\paragraph{Adversary knowledge and approximations}

An \emph{adversary's knowledge} (see \S\ref{sec:security}) is the set of
all possible secret values that are consistent with the attacker's
observations. The adversary starts off with the set of all possible
secrets as they have not made any observations by running queries.
When the adversary observes a new result, their knowledge is
refined by discarding those secrets that are not consistent with the new
observation. For instance, consider that the secret is a natural number
$n$. Initially, an adversary does not have any information about
$n$, so they considers all natural numbers as possible, that is, her
knowledge is the set $\mathbb{N}$. If later the adversary executes the
query $n\ \texttt{mod}\ 3 = 0$ and learns the result is true, then the
attacker knows that the secret is a multiple of $3$, i.e., her knowledge is now refined to
$\{ n \in \mathbb{N} \mid \exists k.\ n = 3k\}$. 


Precisely representing and deriving an adversary's knowledge is, in
general, an uncomputable task. To overcome this, one can approximate the
knowledge using an abstract domain.
% compute sound
% and complete approximations of the knowledge, which we informally
% describe next and formalize in \S\ref{??}.
An \emph{abstract domain} \adom represents a set of secrets that allow
us to reason about the entire set of secrets together.
% takes as input (1) the current
% (approximated) knowledge, (2) the secret information, and (3) the
% current computation, and it outputs the updated approximated knowledge.
Informally, we say our approximation is \emph{under-approximate} whenever the
output knowledge is a subset of the actual knowledge. 
That is, a \emph{under-approximation} ensures that any secret that is
possible according to the approximation also belongs to the actual
knowledge. An under-approximation, therefore, provides a lower-bound on the
attacker's uncertainty with respect to the secret. Similarly, the
approximation is \emph{over-approximate} whenever the approximate knowledge is a
super-set of the actual knowledge. That is, if a secret is not
consistent with an over-approximation, then it is not consistent with
the actual knowledge either. An over-approximation, thus, provides an
upper-bound on the attacker's uncertainty with respect to the secret.

% \mg{I'm not sure I like sound/complete. Perhaps under/over-approximation is better?}

Figure~\ref{fig:ship-spec} shows th

\paragraph{Example}
%
Consider a data owner that wants to protect its location, which we represent as a pair \verb!<x,y>! of coordinates.
%
The data owner, however, would like to selectively allow third-party services to run computations on her location data, for instance for showing targeted advertisements for the closest coffee shop.
%
For this, she will analyze all third-party computations to check how they affect a potential attacker's knowledge to prevent, for instance, her location to be identified too precisely.
%

\sng{push the above to intro?}


\subsection{Posterior Generation by Example}
\todo{add a diagram with the components of the tool with references to each section}

We present by example \tool, 
a framework that given a function on a concrete domain 
computes a correct-by-construction posterior 
on a specified abstract domain.

\begin{figure}
\centering
\begin{subfigure}[b]{0.48\textwidth}
\includegraphics[scale=0.65]{sound.pdf}
\caption{sound posterior}
\label{fig:nearby-sound}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.48\textwidth}
\includegraphics[scale=0.65]{complete.pdf}
\caption{complete posterior}
\label{fig:nearby-complete}
\end{subfigure}
\caption{nearby example \sng{change colors above}}
\label{fig:nearby-example}
\end{figure}

\paragraph*{Problem}

Consider a simplified version of one of our benchmarks: the \emph{Ships}
problem. Here the secret is the location of the ship @Loc@
specified by its @x@ and @y@ coordinates. \mg{Is it simplified?}

\begin{code}
  data Loc = Loc { x :: Int, y :: Int}
\end{code}

Suppose that a user wants to execute a @nearby@ query to answer if the ship's location is
within 100 distance units of the (200, 200) coordinate, measured using Manhattan distance.

% \paragraph{User Input: Query on a Concrete Domain}
% \tool comes with some predefined concrete domains. 
% For this example, the concrete domain we will use is 
% @Point@, defined in a homonymous library, as 
% a datatype with an @x@ and a @y@
% coordinates: 
% %
% \begin{code}
%   data Point = Point { x :: Int, y :: Int}
% \end{code}

% The user of \tool defines a function can import the @Point@
% library and define functions on points.

% The user can then define a computation of the secret that computes some
% boolean result \sng{put the type annotation?}. For example, the @nearby@
% function checks 
% For example, the @nearby@ function below 
% checks that its input @z@ point is nearby too the @l = (200,200)@
% cordinates by computing that euclidean distance between @l@ and @z@ 
% is not more than @100@. 
\begin{code}
  nearby :: Loc -> Bool
  nearby z = abs (x z - x l) + abs (y z - y l) <= 100
    where
      l = Loc 200 200

  abs :: Int -> Int 
  abs x = if x < 0 then -x else x 
\end{code}

\sng{use same terminologies in Marco's and this text}. 
To understand what information is disclosed by the query, a privacy-concerned data owner  starts from the prior knowledge (induced by prior queries) and estimates the posterior knowledge. 
%
If the query result reveals the ship's location to be within some narrow range
of it's true location, the data owner may choose to not answer the query.


% To construct a sound-by-construction posterior of 
% @nearby@ the user needs to simply 
% add an annotation\footnote{GHC annotations are special comments interpreted by ghc-plugins:
% \href{https://gitlab.haskell.org/ghc/ghc/-/wikis/annotations}{https://gitlab.haskell.org/ghc/ghc/-/wikis/annotations}} 
% to the code. 
% The annotation below requests \tool
% to generate a sound-by-construction posterior of the function @nearby@
% with respect to the @Rectangle@ abstract domain. 
% \begin{code}
%   {-# ANN module ("sound", "nearby", "Rectangle") #-}
% \end{code}

\paragraph*{The Range Abstract Domain}

The Range abstract domain $[a, b]$ can be used as an abstraction $A$ for an
integer value $i$ whose lower bound $a$ and upper bound $b$ are known.
% The abstraction $[a, b]$ is a sound abstraction of $i$ iff $a \leq i \leq b$. 
The abstraction $[a, b]$ represents all values  $i$ such that  $a \leq i \leq b$. 
%
We will represent the knowledge of the user $U$ running the query
in form of intervals. We define some operators on these beliefs, such
that we can treat ranges as an abstract domain \sng{not sure if
introducing formal definitions here is a good idea}:
$$
\begin{array}{rcl}
i \in [a, b] & ::= & a \leq i \land i \leq b\\

[a_1, b_1] \subseteq [a_2, b_2] & ::= & a_2 \leq a_1 \land b_1 \leq b_2\\

[a_1, b_1] \cap [a_2, b_2] & ::= & [max(a_1, a_2), min(b_1, b_2)]\ \textnormal{if}\ a_2 \leq b_1
\end{array}
$$
\mg{$\cap$ is undefined if $a_2 > b_1$?}

\mg{What does it mean being a ``sound abstraction''? } 
\mg{Here we keep mixing knowledge and abstract domains (e.g., operators on beliefs). I'd probably simply stick to abstract domains here.}
% Thus for example, the if the ship is at $178$ x-coordinate then the 
% interval $[100, 200]$ is a sound abstraction for it. 
In order to model knowledge about @Loc@ we need to
lift both the x and y coordinate to the Range abstract domain, as the
@LocRange@ datatype:

\begin{code}
  data IntRange = IntRange { lower :: Int, upper :: Int}
  data LocRange <p :: Loc -> Bool, n :: Loc -> Bool> = LocRange {
    xr :: IntRange
  , yr :: IntRange }
\end{code}

The @LocRange@ datatype allows us to model the knowledge for
the location of the ship. When expressed graphically, the location of
the ship is a point while the belief is a rectangle.
Both the outer boxes @B@ shows in Figure~\ref{fig:nearby-example} shows
the initial belief of the user. The @LocRange@ datatype is parameterized
by two predicates to denote the elements it contains. The @p@ property
satisfies all elements that belong to @LocRange@, while @n@ describes all
elements that lie outside @LocRange@.

The exact definition of abstract
refinements~\citep{abstract-refinements} is provided
in~\S~\ref{sec:encoding}. 
Indexing the abstract domain with 
the positive and negative predicates allows us to semantically reason 
about the abstract domains decidably and without the need 
to perform type level operations about \textit{each} element of the domain.

If we plot all the points for which the @nearby@ query will answer
@True@ they will all be within the diamond in both the figures of
Figure~\ref{fig:nearby-example}. Likewise, all the points outside the
diamond will represent the inputs for which @nearby@ query will be
@False@. There is no way to represent the diamond exactly using the
@LocRange@ datatype. This is the key concern with static
analysis, there is no way to precisely represent an abstraction in the
domain used in the analysis. Thus, we either find an underapproximation
(ie. a sound approximation)---an abstraction where all concrete
values satisfy the property or an overapproximation (ie. a complete
approximation)---an abstraction that contains all points that satisfy
the property.

\mg{This repeats the point we already made before. We need to make a pass and consolidates story and terminology.}

% \paragraph{The Rectangle Abstract Domain}
% %

% \sng{this paragraph can go? proof terms originate because of
% intersection, so can we omit that from overview and more that in later
% section?}
% A rectangle is defined by \tool as a datatype that is indexed~\citep{abstract-refinements}
% by two predicates of the points it contains: 
% \begin{mcode}
%   data Rectangle <pos::Point -> Bool, neg::Point -> Bool>
% \end{mcode}
% the @pos@ property captures a property that all the points 
% that belong on the rectange satisfy, while @neg@ describes a 
% property that all elements outside of the rectange. 
% %
% As an example, below we present three trivial rectangles: 
% the empty, the full, and the start. 
% %
% \begin{mcode}
%   type Empty = Rectangle <{\p -> False, \p -> True}>
%   type Full  = Rectangle <{\p -> True, \p -> False}>
%   type Start = Rectangle <{\p -> p=Point 0 0, \p -> p /= Point 0 0}>
% \end{mcode}
% %
% @Empty@ contains no points, so all points it contains satisfy the predicate @False@
% and all not contained satisfy @True@. 
% The dual holds for the @Full@ domain. 
% These predicates can refer to the points, for instance @Start@
% only contains the point @(0,0)@, so the positive predicate 
% is an equality and the negative a disequality with this exact point. 

% The exact definition of Rectangle is provided in~\S~\ref{sec:encoding}. 
% Here we note that indexing the abstract domain with 
% the positive and negative predicates, allows us to reason 
% about the abstract domains deciidably and without the need 
% to perform type level operations about \textit{each} element of the domain. 


\paragraph{Encoding of the Sound Posterior}

The belief represents the set of possible secrets that the user believes
the secret can be in. The execution of the query can only reveal more
information about the secret - thus allowing the user to refine their
belief. If the @nearby@ query returns @True@, then the user can narrow
their initial belief down to the region inside the diamond. Thus any
belief that can be represented as a rectangle inside the diamond is a
sound belief after the execution of the query. Put in other words, all
points inside the posterior belief rectangle should evaluate to True
under the nearby function. If a query returns False, a sound posterior
belief will be any rectangle domain outside the query diamond. Thus any
point in this rectangle should evaluate on the nearby query to False. 

Thus, a sound posterior with respect to the @nearby@ function and a
secret value @secret@ is a rectangle whose elements agree with the
response of @nearby secret@. The refinement type of a function that
produces the sound posterior will be:
%
\begin{mcode}
  {-@ sound :: secret: Loc
    -> {prior: LocRange | secret $\in$ prior}
    -> {post:  LocRange<{p:Loc | nearby secret <=> nearby p},{\_ -> True}|post $\subseteq$ prior> 
  @-}
\end{mcode}

Notice that the final posterior belief depends on the prior belief
because it is a subset of the prior belief. The type signature of
@sound@ uses @True@ as the negative predicate
(\ie we know nothing about the elements outside of the posterior)
but captures soundness on the positive predicate by stating that 
all points in the posterior agree with @nearby@ on @secret@.

We can now try to implement the sound function and get it verified by
LiquidHaskell. If we try to come up with an expression that computes the
posterior, it would look something like this \sng{this is not valid
haskell, because of the last line?}:

\begin{mcode}
  case (nearby secret) of
    True  -> LocRange (IntRange (max xl 188) (min xu 212))
                      (IntRange (max yl 112) (min yu 288))
    False -> LocRange (IntRange (max xl 301) (min xu 500))
                      (IntRange (max yl   0) (min yu 500))
  where
    prior = LocRange (IntRange xl xu) (IntRange yl yu)
\end{mcode}

Writing this function is difficult for two reasons.
First, we need to come up with a sound integers, which normally 
implies solving tedious arithmetic. Second, even after solving for all
these constants, we only have a partially correct implementation. This
implementation does not actually check that the ranges are well formed,
\ie the lower bound is less than or equal to upper bounds. This leads
buggy solutions that do not get verified by LiquidHaskell. \sng{should
we elaborate more on the difficulty?}

\mg{What are sound integers?}

\paragraph{Synthesizing the posterior domains}

To mitigate this challenges, \tool can synthesize the sound posterior
presented in the example above. The key insight \tool uses is to split
the synthesis problem into a simpler problem, by producing a query
specific rectangle $\mathcal{A}_q$, but independent from the prior
belief, then the final solution to the problem can be written as @prior@
$\cap\ \mathcal{A}_q$. \sng{should we frame this as component based
synthesis?} The $\mathcal{A}_q$ can be found by solving the
constraints $\exists \mathcal{A}_q \forall c. c \in \mathcal{A}_q
\implies \textrm{nearby}\ c$ when the result of the query is True. When
the result of the query is false, $\mathcal{A}_q$ can be found be solving
$\exists \mathcal{A}_q \forall c. c \in \mathcal{A}_q \implies
\lnot(\textrm{nearby}\ c)$. The intersection operation makes sure that
the result is a subset of the prior and the implication ensures that all
points inside our domain satisfies the constraints from the query.

\mg{Is the key insight really that we can split the problem? 
%
My feeling was that the key insight is the encoding (which enable decidable reasoning) and which we do not stress too much so far.}

\tool accepts a list of bounds in which the belief can belong and then
solves for the bounds of $\mathcal{A}_q$. This means the user just needs
to input only the bounds and the query function over the secret
datatype, the rest are synthesized by \tool. The final posterior
expressions are synthesized along with their refinement types so that
the solutions can be verified end to end with LiquidHaskell.

\sng{move all example code to a figure to omit repetation of code}

\tool is a GHC plugin, that works on valid Haskell source programs and
takes additional input as source annotations:

\begin{mcode}
data Ship = Ship {
  capacity :: Int,
  x        :: Int,
  y        :: Int
}
{-# ANN Ship ([
  ("capacity", (0, 100)),
  ("x", (0, 500)),
  ("y", (0, 500))
  ] :: [(String, (Int, Int))]) #-}

{-@ reflect abs @-}
abs :: Int -> Int
abs i | i < 0 = -1 * i
abs i         = i

{-@ reflect query @-}
query :: Ship -> Bool
query secret = (capacity secret) > limit && (abs (x secret - 200) + abs (y secret - 200) <= d)
  where
    limit = 50
    d = 100

{-# ANN module ("sound", "query") #-}
{-# ANN module ("complete", "query") #-}

\end{mcode}

Here the @ANN@ for the datatype @Ship@ refers to the minimum and maximum
bounds for the beliefs of each field in the secret. The last two @ANN@s
say that we want \tool to generate a \emph{sound} underapproximation and
a \emph{complete} overapproximation for the query. \tool GHC plugin runs
as a part of a Haskell compiler and produces a separate file with all
the approximations as requested. This file can be verified against the
query by LiquidHaskell or can be manually inspected and modified by the
user to include other approximations as deemed fit. In practice, often
it is more useful to produce an approximation that is balanced along all
dimensions. \tool uses Z3 inbuilt optimization support to produce such
an approximation.

\begin{mcode}
{-@ soundHelper :: secret: Secret
       -> {prior: Range | secret $\in$ prior}
       -> Range<{l:Secret | nearby secret <=> nearby l}, {\_ -> True}> 
@-}
soundHelper :: Secret -> Range -> Range
soundHelper secret _ = case (nearby secret)  of
  True  -> LocRange (IntRange 188 212) (IntRange 112 288) -- proof terms omitted
  False -> LocRange (IntRange 301 500) (IntRange   0 500) -- proof terms omitted
\end{mcode}

In~\S~\ref{sec:synthesis} we explain how we used SMT's synthesis and 
optimiziation features to encode and synthesize correct posteriors. 
Second, we need to come up with boiler-plate proof terms 
that the rectangular satisfies the property indexes.
In~\S~\ref{sec:implementation} we describe how we mechanised the 
synthesis of such boilterplate code, using metaprogramming of GHC's plugin. 

As a last step, the sound posterior is intersected with the prior
\begin{mcode}
-- same liquid type for sound as shown above
sound :: Secret -> Range -> Range
sound secret prior = prior $\cap$ soundHelper secret prior
\end{mcode}

% \paragraph{Monotoniicity of the postperior}
% In practise \todo{for reasons that Marco explained above}, we require that 
% each derived function computes a posterior 
% that is a subset of our prior (\ie the current knowledge). 
% Our @Rectangular@ abstract domain library defines operator that 
% combine abstract domains. 
% For instance, below we @intersect@ the above @soundPost@ abstract domain 
% with the current prior: 
% %
% \begin{mcode}
%   {-@ sound :: secret: Point
%     -> {prior: Rectangle | secret $\in$ prior}
%     -> {post:Rectangle<{l:Point | nearby secret <=> nearby l}, {\_ -> True}> | post $\subset$ prior  }
% @-}
%   sound secret prior = prior `intersect` soundPost secret prior 
% \end{mcode}
% %
% In~\S~\ref{sec:encoding} we present the definition of @intersect@
% and how it is specified to provably intersect the positive and negative indices 
% of the rectangular domain. 


\paragraph{Encoding of the Complete Posterior}
Dually, we user can request the derivation of a complete posterior. 
In this case, \tool will generate the below complete posterior.
\begin{mcode}
  {-@ completeHelper :: secret: Secret
       -> {prior: Range | secret $\in$ prior}
       -> {post:Range<{\_ -> True}, {l:Secret | $\lnot$(nearby secret <=> nearby l) $\lor$ $\lnot$(l $\in$ prior) }> | true }
@-}
completeHelper :: Secret -> Range -> Range
completeHelper secret _ = case (nearby ) 
  True  -> LocRange (IntRange 100 300) (IntRange 100 300) -- proof terms omitted
  False -> LocRangeFull                                   -- proof terms omitted
\end{mcode}
The positive predicate of a complete return posterior is true, \ie 
we know nothing about the elements that belong to the posterior. 
But, the negative predicate states that either the elements do not comply 
with the secret on nearby of they did not belong to the original prior. 
Once again, \tool synthesizes the definition of a complete posterior. 
In this case, it returns a function that when @nearby secret@ is true 
returns the rectangular @(100,300)x(100,300)@ 
(\ie a rectangular that contains the @nearby secret == True@ response), 
otherwise, it returns a ``full'' rectangular (\ie any point can belong to the posterior).


As a last step, the complete posterior is intersected with the prior.
\begin{mcode}
  {-@ complete :: secret: Loc
  -> {prior: LocRange | secret $\in$ prior}
  -> LocRange<{\_ -> True}, {l:Loc | $\lnot$ (nearby secret <=> nearby l) $\lor$ $\lnot$ (l $\in$ prior) }>
@-}
  complete secret prior = prior $\cap$ completeHelper secret prior
\end{mcode}


\subsection{Summary}
\tool comes with predefined concrete and abstract domains and automatically 
derives correct-by-construction posteriors of user defined functions. 
We used \tool on \todo{menion the concrete and abstract domains we have}
and in~\ref{sec:evaluation} we evaluate our technique. \sng{change this
after writing whole paper?}

==> overview.tex <==
\section{Overview}
\label{sec:overview}

We start off with a representative task for web apps that
operates over sensitive user data: showing ads based on the location of
the user, and demonstrating how such a verified system can be
written in \tool. We present the example in conjunction with
LIO~\cite{stefan2011flexible}, a Haskell library to enforce
non-interference, and show \tool composes well with other security
monads. \sng{forward reference to next few subsections}

\begin{figure}
\begin{mcode}
data UserLoc = UserLoc { x :: Int, y :: Int}

nearby :: UserLoc -> Bool
nearby UserLoc {..} = abs (x - 200) + abs (y - 200) <= 100 where abs i = if i < 0 then -i else i

policy :: ADom -> Bool
policy dom = size dom > 100

type ALIO = AnosyT ADom (Labeled DCLabel UserLoc) (LIO DCLabel)

getUserLocation :: String -> LIO DCLabel (Labeled DCLabel UserLoc)

nearbyL :: Labeled DCLabel UserLoc -> Bool
nearbyL (LabeledTCB _ s) = nearby s

showAd :: String -> ALIO Bool
showAd name = do
  secret <- lift (getUserLocation name)
  modify (*\$*) \s -> s { secret = Just secret }
  downgrade nearbyL underapprox

underapprox :: p: ADom -> 
  (ADom <{\x ->   nearby x && (x $\in$ p)},{\_ -> True}>,
   ADom <{\x -> $\lnot$ nearby x && (x $\in$ p)},{\_ -> True}>)
underapprox p = (p $\cap$ trueInd, p $\cap$ falseInd)
  where (trueInd, falseInd) = under_indset

under_indset::(ADom<{\l ->   nearby l},{\_ -> True}>,
               ADom<{\l -> $\lnot$ nearby l},{\_ -> True}>)
under_indset = ((ADom (Interval 121 279)
                      (Interval 179 221)),
                (ADom (Interval   0 400)
                      (Interval   0  99)))
\end{mcode}
\caption{Definition of the secret, query and security policy.}
\label{fig:userloc-defn}
\end{figure}

% \sng{Ideas: Show a complete example around underapprox showAd function,
% and step by step how one would go about writing the program in \tool.
% This means connect each subsection step-by-step. Show the minimal needed
% interface for Anosy and how to fill in required functions, and
% synthesize those posteriors. Will cut the overapprox and free space
% while giving us an idea of how Anosy works in practice in a full problem.}

Suppose a restaurant chain wants to
show ads to a user if the user is near any of their restaurants.
The chain selects a criteria that if the user is in 100 units of
distance from a restaurant location, then an advertisement will be shown
for that location. Figure~\ref{fig:userloc-defn} shows the definitions
of the data types and related functions. Consider a user, whose location
is represented with the @UserLoc@ data type, using the
@x@ and @y@ fields to encode the coordinates. The @nearby@ function
shows an example query when a restaurant located at the (200, 200)
coordinate wants to show ads to users within 100 units of Manhattan
distance. Execution of this query leaks information whether the user is
in the expected location range. Similarly, other locations of the chain
will also query the user with their location, to 
determine if an advertisement should be shown for that branch.
However, when the restaurant chain combines the learned information
about the user's location for each query, they might infer a precise
estimate of the user's exact location.
% \nv{word restaurant appears tooooo many times :)}
% \sng{reduced a few, check if ok}
Running computations on secret data reveals information about the
secret, causing data leaks. The key problem arises from the ability to
run multiple different queries on a secret without any policies to
safeguard how much information a third-party is allowed to learn about
the secret. With such a policy for limiting information leakage in place, the
advertisement platform can maximize the number of advertisements they
can show, while still providing security guarantees.

The @policy@ function shows a sample security policy.
% \nv{why talk about prior and posterior here? say directly the last sentence}
The @ADom@ type represents a set of user locations the adversary
considers possible.
% We assume an adversary starts off with a belief of all possible user
% locations, also known as \emph{prior} knowledge. As the adversary runs
% more queries, they get a better estimate of the user's location. In
% other words, they refine their prior knowledge to get a \emph{posterior}
% knowledge. We discuss these in details in \S~\ref{subsec:indset}.
% The policy says, a third-party can
% view the result of the query only if the abstract domain represents more
% than 100 possible user locations, irrespective of the whether the
% query returns @True@ or @False@.
The @size@ function (definition
omitted) computes the number of concrete secrets inside the abstract
domain. In other words, the policy specifies in no circumstance can a
third-party be allowed to narrow the user's location to a set of 100 or
fewer locations.

The @ALIO@ type is constructed by composing the @AnosyT@ monad
transformer with the @LIO@ monad. The type denotes a @AnosyT@
computation wrapping a @LIO@ computation that estimates the set of
secrets using @ADom@ type, and the secrets are labeled instances of the
@UserLoc@ type. These labels are used by @LIO@ to check information flow.
While the @AnosyT@ monad can be composed with any monad, our use of
@LIO@ is an example to show how quantitative information policies can be
used with non-interference for safe declassification.

The @getUserLocation@ function (definition omitted), given an username
retrieves the user location and labels the data with the username, to
ensure that only permitted functions can read the private user data.
@nearbyL@ is the function that does the declassification: it takes a
labeled location, and runs the @nearby@ query while ignoring the label.
The goal is to wrap this computation with a policy, so that we have
guarantees about the amount of information leaked.

The @showAd@ function combines these primitives in a safe manner.
It uses @downgrade@ (provided by \tool) to execute the @nearbyL@ query if
it deems safe to run with respect to the policy. The @ALIO@ return type
returns an computation that evaluates to the value of the query or an
error if the declassification is unsafe. A sequence of such @downgrade@s
can be used track the information leakage over multiple queries.

% \sng{need to mention size is 400x400 and describe the steps in AIO type
% and showAd function and what is OverApprox}

% \begin{figure}
% \begin{mcode}
% downgrade :: (UserLoc -> Bool) -> ADom
%           -> (ADom -> Bool) -> UserLoc -> Bool
% downgrade query prior policy secret =
%   let (tPost, fPost) = over_post prior over_indset in
%   if (policy tPost) && (policy fPost)
%   then query secret
%   else userError "unsafe operation"
% \end{mcode}
% \caption{Definition of \texttt{\textbf{downgrade}}.}
% \label{fig:downgrade-defn}
% \end{figure}

% Figure~\ref{fig:downgrade-defn} defines the
% \texttt{\textbf{downgrade}} operation that allows us to safely
% declassify sensitive computations. \sng{fix me}

% The @AnosyT@ monad transformer allows us to compose \tool with with other
% security monads, such as LIO~\cite{stefan2011flexible} (to enforce
% \emph{non-interference}), to track the secret, policy, and knowledge of
% an attacker. In our example, we use the @AnosyT@
% transformer to make a bare minimal @AIO@ monad.
% Running a query over the secret computes all possible posteriors (for
% each return value of the query), and if none of posteriors violate the
% policy executes the query else throws an error. Our running example uses
% over-approximations to estimate the information leaks.
% The function @over_post@ computes the posterior knowledge given a
% prior knowledge about the secrets, and the value @over_indset@
% is the \indset for the query. We elide both these definitions here, but in
% the following sections, we will present how \tool aids in writing
% correct definitions for the \indsets and the posteriors. Note, that
% computing the posterior for a sequence of computation would require the
% programmer to track the adversary knowledge as it evolves through
% multiple queries. However, in practice, \tool{} lifts all computations
% to a monad @AnosyT@ to automatically track the adversary

\nv{Indeed too much info, we should abstract away all the LIO info here
to make this work} \sng{fixed now! can you check?}

In the following sections, we will discuss how one would write the
posterior definitions and verify these with \tool.

\subsection{Approximating knowledge from queries}
\label{subsubsec:knowledge}

\begin{figure*}
\centering
\begin{subfigure}[b]{0.33\textwidth}
  \centering
  \includegraphics[width=0.7\textwidth]{ship-real-bw}
\caption{Indistinguishability Sets}
\label{fig:nearby:real}
\end{subfigure}%
\begin{subfigure}[b]{0.33\textwidth}
  \centering
\includegraphics[width=0.7\textwidth]{ship-under-bw}
\caption{Under-Approximation}
\label{fig:nearby:under}
\end{subfigure}%
\begin{subfigure}[b]{0.33\textwidth}
  \centering
\includegraphics[width=0.7\textwidth]{ship-over-bw}
\caption{Over-Approximation}
\label{fig:nearby:over}
\end{subfigure}
\caption{Indistinguishability Sets and their
Rectangular Approximations with respect to \texttt{nearby} query.
\sng{change to vector art}}
\label{fig:nearby-example}
\end{figure*}

The \emph{knowledge} of an attacker evolves as they observe more results
from the execution of queries~\cite{askarov2007gradual}.
For example, the attacker might already have some prior knowledge about the user's 
location and might use the result of the @nearby@ query to refine this
knowledge. However, precisely computing and representing attacker
knowledge requires reasoning about all points in the input space, an
uncomputable task in general. Abstract domains such as
intervals~\cite{cousot1976static}, octagons~\cite{mine2006octagon}, and
polyhedra~\cite{cousot1978automatic} 
reason about sets of program states and can be used to approximate
knowledge. While we use an under-approximation with intervals in this
example, \tool supports both \textit{under-approximations} and
\textit{over-approximations} of the attacker knowledge over multiple
abstract domains.


\paragraph{Indistinguishability sets}

The @nearby@ boolean query partitions the space of secrets into
two partitions (for 2 possible responses: @True@ and @False@), called
\textit{indistinguishability sets} (\indsets), 
\ie all secrets in each partition produce the same result for the
@nearby@ query. Figure~\ref{fig:nearby:real} depicts the two \indsets 
for the @nearby@ query. The inner diamond---depicted in light
gray---is the \indset for the result @True@, \ie all its elements
respond @True@ to the @nearby@ query. In contrast, the
outer region---depicted in dark gray---is the \indset for
@False@. The @under_indset@ function defines the
under-approximate \indsets for the @nearby@ query. It 
is a tuple, where the first element corresponds to the
@True@ response, and the second element to the @False@ response. It says
all secrets in $x \in [121, 279]$ and $y \in [179, 221]$, evaluates to
@True@ for the query, and all secrets in $x \in [0, 400]$ and $y \in [0,
99]$ evaluates to @False@. The refinement type signature for
@under_indset@ verifies this. We discuss this in more detail in
\S~\ref{} \sng{ref}.


% The
% refinements on @under_indset@ type states that 
% for the first element in the tuple, all secret @UserLoc@
% inputs represented by the abstract domain evaluate to @True@ for
% @nearby@. Similarly for the second element of the tuple, all
% @UserLoc@ elements represented by the abstract domain, it
% evaluates to @False@. Using the @ADom@ abstract domain, we can write
% under-approximation of the \indsets for the @nearby@ query as follows:

\paragraph{Knowledge under-approximation.}

To compute the possible \emph{posterior} knowledge after the query, \ie
the set of states the attacker considers possible,  
we simply take the intersection $\cap$ of the prior knowledge with the
\indset associated with the query~\cite{askarov2007gradual,
backesleak09}. If the intersection happens with the exact \indsets, then
we derive the exact posterior. For our example, we intersect with the
under-approximate \indset to produce an under-approximation of the
posterior knowledge \ie a lower-bound on the information learned by an
attacker when observing the query result. The intersection $\cap$ refers 
to the set-theoretic intersection of two domains. We formally define
these operations in \S~\ref{sec:encoding}.

The refinement type states, an under approximated posterior knowledge is
an abstract domain (@ADom@) whose elements agree with the
response of @nearby@ and belongs to the prior knowledge
@p@ of the adversary. The tuple of @ADom@ represents the abstract domain
for both @True@ and @False@ response of the query respectively and take
element-wise intersection $\cap$ with @under_indset@. \nv{add forward
reference}

LiquidHaskell can mechanically prove that the provided values for the
under-approximation are correct for the @nearby@ query at compile time.
\sng{talk about omitting proof terms?}
% In other words, Liquid Haskell mechanically 
% proves that the returned abstract user location domain is an under-approximation
% of @nearby@'s \indset. % for the given secret input 

% \paragraph{Knowledge over-approximation.}

% Dually, we can write an over-approximate posterior  
% as the intersection of prior with the over-approximate \indsets. 

% \begin{mcode}
% over_post :: p: ADom ->
%   (ADom <{\_ -> True},{\x -> (*$\lnot$*) nearby x (*$\lor$*) (x (*$\not \in$*) p)}>,
%    ADom <{\_ -> True},{\x ->   nearby x (*$\lor$*) (x (*$\not \in$*) p)}>)
% over_post p = p (*$\cap$*) over_indset
% \end{mcode}

% The specification of @over_post@ % encodes completeness since it 
% uses the negative index predicate to specify properties about all points
% excluded from the abstract domain.
% The first @ADom@ excludes all @UserLoc@s that are
% either not @nearby@ or outside the prior. Similarly, the second
% @ADom@ excludes all @UserLoc@s that are
% either @nearby@ or outside the prior.

% \subsection{Modeling Indistinguishability Sets}
% \label{subsec:indset}



% Precisely computing and representing attacker knowledge requires
% reasoning about all points in the input space, an uncomputable task in
% general. Abstract domains such as intervals~\cite{cousot1976static},
% octagons~\cite{mine2006octagon}, and
% polyhedra~\cite{cousot1978automatic} 
% reason about sets of program states and can be used to approximate
% knowledge. While we use an under-approximation with intervals in this
% example, \tool supports both \textit{under-approximations} and
% \textit{over-approximations} of the attacker knowledge over multiple
% abstract domains.

% Figure~\ref{fig:nearby:under} shows an \textit{under
% approximation} of @nearby@'s \indsets.
% The light gray region in Figure~\ref{fig:nearby:under} is a
% subset of the  precise \indset for the @True@ result (light gray
% region in Figure~\ref{fig:nearby:real}). 
% To be an under approximation, all elements in the abstract domain 
% must be a member of the \indset. 
% Similarly, the dark gray region in Figure~\ref{fig:nearby:under} is a
% subset of the precise \indset for the @False@ result (dark grey region
% in Figure~\ref{fig:nearby:real}).

% The @nearby@ boolean query partitions the space of secrets into
% two partitions (for 2 possible responses: @True@ and @False@), called
% \textit{indistinguishability sets} (\indsets), 
% \ie all secrets in each partition produce the same result for the
% @nearby@ query. Figure~\ref{fig:nearby:real} depicts the two \indsets 
% for the @nearby@ query. The inner diamond---depicted in light
% gray---is the \indset for the result @True@, \ie all its elements
% respond @True@ to the @nearby@ query. In contrast, the
% outer region---depicted in dark gray---is the \indset for
% @False@. \Indsets are used to track an attacker's
% knowledge~\cite{askarov2007gradual, backesleak09}, \ie the set of states
% the attacker considers possible, over multiple queries.
% % \footnote{The information leaked by a program is often formalized using an
% % equivalence relation over program states, where equivalent states cannot be
% % distinguished by the attacker~\cite{backesleak09}. We refer
% % to the equivalence classes induced by the relation, where each \indset
% % is one of such classes.}
% The knowledge can then be used to characterize
% the information leaked through each computation, thus helping the design
% of security policies.


% For @nearby@, figure~\ref{fig:nearby-example} depicts approximations
% of the \indsets using the interval abstract domain which can be either
% \textit{under approximate} or \textit{over approximate} \indsets.
% Dually, an abstract domain is an \textit{over approximation} when all
% points in it is a superset of the \indset; see
% Figure~\ref{fig:nearby:over} for abstract
% domains over approximating the \indsets from \ref{fig:nearby:real}. 
% We represent abstract domains as data types like the following:

% \begin{mcode}
% data Interval = Interval { l :: Int, u :: Int}
% data ADom <p::UserLoc -> Bool, n::UserLoc -> Bool>
%   = ADom { xr :: Interval, yr :: Interval }
% \end{mcode}

% @Interval@ defines the interval abstract domain for an integer in
% the range between the lower @l@ and upper @u@ fields. 
% @ADom@ defines the abstract domain for the @UserLoc@ data
% type where each field is an interval abstract domain.
% Importantly, the @ADom@ data type is parameterized
% by two predicates to denote the elements it contains. The @p@
% property is satisfied 
% by all secrets that belong to @ADom@, whereas @n@ describes all
% secrets that lie outside @ADom@.
% For example, below we present the types that encode an empty, a full,
% and a domain representing the user located at the origin, by their types.

% \begin{mcode}
% type EmptyADom = ADom <\_ -> False, \_ -> True>
% type FullADom  = ADom <\_ -> True,  \_ -> False>
% type OrigADom  = ADom <\u -> u = UserLoc 0 0,
%                        \u -> u (*$\not =$*) UserLoc 0 0>
% \end{mcode}

% The positive predicate of @EmptyAdom@ states that all its elements
% should satisfy @False@, thus it represents the empty abstract domain.
% Dually, the negative predicate of @FullAdom@ states that all the
% elements that do not belong to the domain should satisfy 
% @False@, thus it represents the full abstract domain.
% Finally, the predicates of @OrigAdom@ state that its elements 
% are exactly equal to @UserLoc 0 0@, which is satisfied only by
% the user that is positioned at the origin of the space. 
% The exact definition of abstract
% refinements~\cite{abstract-refinements}, where it is also parameterized
% over any secret data type. Indexing the abstract domain with 
% these positive and negative predicates allows us to semantically reason 
% about the abstract domains decidably, without the need 
% to perform type level operations about \textit{each} element of the domain.

% The abstract domain @ADom@ must implement a set of operations
% (shown below) that, combined with the predicate indexes, lets us specify
% and prove that the approximate \indsets under- or over-approximate the
% real \indsets.

% \begin{mcode}
%   (*$\in$*) ::  UserLoc -> ADom -> Bool 
%   (*$\subseteq$*) :: ADom -> ADom -> Bool 
%   (*$\cap$*) :: ADom -> ADom -> ADom 
% \end{mcode}

% These operators are defined using the standard set-theoretic semantics, \eg
% @UserLoc x y $\in$ ADom (Interval xl xh) (Interval yl yh) = xl $\leq$ x $\leq$ xh $\land$ yl $\leq$ y $\leq$ yh@.

% Figure~\ref{fig:nearby:under} shows under-approximation of
% the \indsets for @nearby@, which is defined by @under_indset@. It 
% \nv{wording is too confusing: try not to use it}
% is a tuple, where the first element is the under-approximation for a
% @True@ response, and the second element when the response is
% @False@. The refinements on @under_indset@ type states that
% for the first element in the tuple, all secret @UserLoc@
% inputs represented by the abstract domain evaluate to @True@ for
% @nearby@. Similarly for the second element of the tuple, all
% @UserLoc@ elements represented by the abstract domain, it
% evaluates to @False@. Using the @ADom@ abstract domain, we can write
% under-approximation of the \indsets for the @nearby@ query as follows:

% \begin{mcode}
% under_indset::(ADom<{\l ->   nearby l},{\_ -> True}>,
%                ADom<{\l -> (*$\lnot$*) nearby l},{\_ -> True}>)
% under_indset = ((ADom (Interval 121 279)
%                       (Interval 179 221)),
%                 (ADom (Interval   0 400)
%                       (Interval   0  99)))
% \end{mcode}

% Dually, figure~\ref{fig:nearby:over} shows the over-approximation of
% \indset as defined by @over_indset@. Here, the negative predicate in the type ensures the domains are
% over-approximations. The first element of the tuple ensures that any
% secrets excluded from the @ADom@ are not nearby, for the query result
% @True@, whereas the second says any secrets excluded should be nearby,
% for the query result @False@.

% \begin{mcode}
% over_indset::(ADom<{\_ -> True}, {\l -> (*$\lnot$*) nearby l}>,
%               ADom<{\_ -> True}, {\l ->   nearby l}>)
% over_indset = ((ADom (Interval 100 300)
%                      (Interval 100 300)),
%                (ADom (Interval   0 400)
%                      (Interval   0 400)))
% \end{mcode}

% It takes an expert to find these bounds for \sng{fix me}
% each query, but we demonstrate how \tool can automate this in
% \S~\ref{subsubsec:anosy:tool}. At compile time, Liquid Haskell
% automatically proves that the provided values for the
% user location abstract domain satisfies this refinement type. \sng{talk
% about omitting proof terms}
% In other words, Liquid Haskell mechanically 
% proves that the returned abstract user location domain is an under-approximation
% of @nearby@'s \indset. % for the given secret input 

\subsection{Automating posteriors using synthesis}
\label{subsec:overview:tool}

Although Figure~\ref{fig:userloc-defn} presents a working example of a
verified program written in \tool, it takes a domain expert to
come up with the integer constants as shown in @under_indset@. While
an incorrect constant will be flagged by verification, there is still a
risk of writing imprecise abstract domains: for example, suppose the
first interval of @under_indset@ definition was written as
@(Interval 121 122)@. Such a domain while correct, represents fewer
secrets than desirable, \ie it is not the tightest lower bound for
under-approximation. This gives an option to the programmer to rely on
synthesis to automate this tedious task, while giving the fallback to
write correct definitions manually if needed.

% \underline{\textsc{A}}pproximate 
% k\underline{\textsc{no}}wledge \underline{\textsc{sy}}nthesizer, which
% \nv{too late to explain the initials... should happen the first time you mention anosy}

To aid in this task, \tool can automatically synthesize under- or
over-approximations of \indsets and 
posterior knowledge for a given query.
\tool's GHC plugin that takes as input annotated Haskell code 
and outputs a Haskell program that includes definitions of the
appropriate approximate \indsets and posterior knowledge.
% that is checked by Liquid Haskell to compute
% knowledge approximations. 
% \jp{LH verifies that the computed posterior distribution is sound/complete, right?}
% In the rest of this section, we present how 
% \tool works on the @nearby@ example. 

% \paragraph{\tool's input: Annotated Haskell Code.}

To use the GHC plugin, we need to add the following annotations to the
source in Figure~\ref{fig:userloc-defn}.

\begin{mcode}
{-# ANN UserLoc ([(   "x", (  0, 400)),
                  (   "y", (  0, 400))]
              :: [(String, (Int, Int))])  #-}
{-# ANN module ("underapprox",  "nearby") #-}
\end{mcode}

The annotation on the @UserLoc@ type states that \tool should bound the
search from 0 to 400 for both @x@ and @y@ fields when synthesizing correct
approximations. The second annotation declare what kind of approximation
(either @underapprox@ or @overapprox@) will be synthesized, and on which
query (@nearby@).

The GHC plugin produces a Haskell source file that contains the @UserLoc@'s
abstract domain definition (@ADom@), and an under-approximation of both
the \indsets @under_indset@ and posterior knowledge @underapprox@, along
with their refinement types, as presented in the previously. These
auto-generated definitions can be used as-is in the @downgrade@ call with
the @showAd@ function. Further, LiquidHaskell can be used to verify the
correctness of the synthesized definitions as a sanity check.

\paragraph{\tool's Synthesis.}

To generate the output Haskell file, \tool's GHC plugin
combines metaprogramming, program sketching, and SMT-based synthesis. 
First, using metaprogramming, it generates the type specifications of
the functions to be synthesized, using defintions similar to
Figure~\ref{fig:userloc-defn} to generate a
program sketch~\cite{solar2006combinatorial}, \ie a partial program
where only @under_indset@ definition is left as a hole, to be
substituted later. Finally, it reduces the refinement-type
specifications to constraints, and solves them to produce the domain
bounds. So for an abstract domain represented by two intervals for the
location: @ADom[$l_1, u_1$] [$l_2, u_2$]@, we can get the following
constraints from the refinment type signatures. We hand this off to an
off-the-shelf SMT 
solver to get the solution. The first implication below is for the
@ADom@ corresponding to the query response @True@ \aka the first
tuple of the \indset, whereas the second implication corresponds to
the second value of the \indset tuple, \ie the @False@ query response.

\begin{align}
\forall x, y.\ & l_1 \leq x \leq u_1\ \land\ l_2 \leq y \leq u_2 \implies nearby(x, y) \tag{Under-approx, \textsf{True}}\\
\forall x, y.\ & l_1 \leq x \leq u_1\ \land\ l_2 \leq y \leq u_2 \implies \lnot nearby(x, y) \tag{Under-approx, \textsf{False}}\nonumber
\end{align}

However, these constraints have multiple correct solutions, but we would
prefer the tighest bounds wherever possible. This translates to
generating the maximal domain when under-approximating, and minimal
domain when over-approximating. We use Z3~\cite{bjorner2015nuz} as the SMT
solver of choice because it supports these optimization directives to
maximize $u_1 - l_1$ and $l_2 - u_2$ together. Once a model with the integer
assignments for $l_1$, $u_1$, $l_2$, and $u_2$ the GHC plugin lifts this to
Haskell code to produce the @under_indset@ and @underapprox@ definitions shown in
Figure~\ref{fig:userloc-defn} in the output file.

% We defer additional details about synthesis, proof terms that aid
% decidable verification, and how \tool
% generalizes to other domains, such as powersets, to the paper~\cite{guria2021approx}.
% % , 
% % while our 
% \anosy's implementation is extensible, making it generalizable to support
% additional abstract domains. 
% % with further abstraction domains. 



% Consider a ship, whose position is secret, moving in a 400x400 space. % where its position is secret. 
% We represent the ship in Haskell with the following @Ship@ data type, 
% where the fields @x@ and @y@ encode the ship's position. 
% \begin{mcode}
%   data Ship = Ship { x :: Int, y :: Int}
% \end{mcode}
% This representation enables
% queries over the ship's secret position to be written as boolean Haskell functions. 
% For example, 
% the @nearby@ function below 
% takes a @Ship@ as input and 
% queries whether
% its position is within 100 units of the center (200,200):
% \begin{mcode}
%   nearby :: Ship -> Bool
%   nearby (Ship x y) = abs (x - 200) + abs (y - 200) <= 100
%     where abs i = if i < 0 then -i else i 
% \end{mcode}
% The @nearby@ query first uses the ship's 
% @(x, y)@
% position to compute its 
% Manhattan distance from
% @(200,200)@ and then checks whether the distance is less than or equal to @100@. 

% The @nearby@ boolean query partitions the plane in two 
% \textit{indistinguishability sets} (\indsets), 
% \ie sets whose elements cannot be distinguished by 
% observers of
% @nearby@'s result. 
% %
% This means that
% all elements in an \indset agree on their result to the @nearby@ query. 
% %
% % \jp{TODO: Relate back to equivalence relation terminology}
% % 
% % TODO: Move this down to knowledge paragraph.
% % As a result, the larger an \indset is the more uncertain the attacker is about @nearby@'s input and, dually, a small \indset indicates that the attacker's uncertainty is low since there are only few possible elements in the set.
% % XXX
% % 
% \Indsets are used to characterize the information leaked through computations and track an attacker's knowledge~\cite{askarov2007gradual,backesleak09}, \ie the set of states he considers possible, over multiple queries.\footnote{
% The information leaked by a program is often formalized using an equivalence relation over program states, where related states cannot be distinguished by the attacker~\cite{backesleak09}.
% %
% We equivalently refer to the equivalence classes induced by the relation, where each \indset is one of such classes.
% %
% % This view is better suited to write programs handling knowledge.
% }
% % \jp{more elaboration on uses of \Indsets?}
% % \nv{we do not need more elaboration, we need a citation}

% Figure~\ref{fig:nearby:real} depicts the two \indsets 
% for the @nearby@ query.
% % , where 
% % @$\mid \mid \bullet \mid \mid$@ in @nearby@'s definition denotes the Manhattan distance. 
% %
% The inner diamond---depicted in light gray---is the \indset for the result @True@, \ie all its elements respond @True@ to the @nearby@ query.
% %
% In contrast, the outer region---depicted in dark gray---is the \indset for @False@.




% \paragraph{Approximating \indsets using abstract domains}
% %
% Precisely computing and representing \indsets is an uncomputable task in general.
% Abstract domains including intervals~\cite{cousot1976static}, octagons~\cite{mine2006octagon}, 
% and polyhedra~\cite{cousot1978automatic}
% reason about sets of program states and
% can be used to approximate \indsets. 
% % ... interval constraints have the form a <= X <= b for program variables X and constants a and b
% %
% % Approximating \indsets using abstract domains
% % \paragraph{Approximations of \indsets}
% % As an example, consider 
% % For the \indsets induced by @nearby@, 
% For @nearby@, 
% \Cref{fig:nearby-example} depicts approximations of the \indsets using the interval abstract domain. 
% Abstract domains 
% can \textit{under approximate} or \textit{over approximate} 
% % the 
% \indsets. 
% % 
% % Figure~\ref{fig:nearby-example} approximates the \indsets induced by @nearby@
% % using the interval abstract domains. 
% The abstract domains in 
% \Cref{fig:nearby:under} 
% % depicts an 
% are an
% \textit{under approximation}
% of @nearby@'s \indsets.
% The light gray interval abstract domain in \Cref{fig:nearby:under} is a subset of the \indset for the @True@ result, which is 
% the light gray set in \Cref{fig:nearby:real}. 
% %
% % where each query result is mapped to a rectangular space that is a subset of the original \indset for the result.
% %
% % That is, 
% To be an under approximation, all elements in the abstract domain 
% % representing an under approximation of the \indset
% must be a member of the \indset. 
% % 
% % under approximations ensure that each point that belongs to the under-approximated \indset for some result $r$ also belongs to the corresponding original \indset for the same result. 
% % 
% Similarly, the dark gray abstract domain in \Cref{fig:nearby:under} is a subset of the \indset for the @False@ result so it is an under approximation of the dark grey \indset in \Cref{fig:nearby:real}.
% % 
% % in which each rectangular space is a subset of the original
% % yes-or-no spaces. 
% % %
% % An under-approximation
% % in general ensures that any secret (here, the location of the ship) that is
% % possible according to the approximation also belongs to the actual
% % \indset. 
% %
% % TODO: Move this down to knowledge paragraph.
% % Therefore, under-approximations provide a lower-bound on the
% % information learned by an attacker by observing the query result.
% % XXX
% %
% % , \ie  two points that are indistinguishable with respect to the under-approximation are so also with respect to the original \indsets. 
% %
% Dually, an abstract domain is an \textit{over approximation} when it is a superset of the \indset; see Figure~\ref{fig:nearby:over} for abstract domains over approximating the \indsets from \Cref{fig:nearby:real}.
% % Figure~\ref{fig:nearby:over}, dually,  depicts an \textit{over approximation}
% % of the \indsets, where each query result is mapped to a rectangular space that is a superset of the original \indset for the result. 
% %
% % TODO: Move this down to knowledge paragraph.
% % That is,  over-approximations provide an
% % upper-bound on the attacker's uncertainty with respect to the input:
% % all inputs that do not belong to the over-approximated \indset do not belong to the original \indset.
% % XXX

% % \mg{I still find this confusing. A query induces two \indsets: one for True and one for False.
% % An approximation also ``induces'' two approximated \indsets: one for  True and one for False. 
% % Make this explicit as `query induces function from query results to subsets of space (that form a partition)' and `approximation is a function from query results to abstract domain'?}
% % \jp{Is that clearer? I split up the \indset for each query result to be more explicit}

% % \jp{TODO}
% % ... Representing abstract domains in Haskell ... LH to mechanically verify over/underapproximations
% We represent abstract domains as data types like the following:
% \begin{code}
%   data Interval = Interval { lower :: Int, upper :: Int}
%   data AShip <p :: Ship -> Bool, n :: Ship -> Bool> = 
%          AShip { xr :: Interval, yr :: Interval }
% \end{code}
% @Interval@ defines the interval abstract domain for an integer in the range between the @lower@ and @upper@ fields.
% @AShip@ defines the abstract domain for the @Ship@ data type where each field is an interval abstract domain. 
% Importantly, the @AShip@ data type is parameterized
% by two predicates to denote the elements it contains. The @p@ property is satisfied
% by all elements that belong to @AShip@, whereas @n@ describes all
% elements that lie outside @AShip@.
% For example, below we present the types that encode an empty, a full, and the origin 
% ship abstractions. 
% \begin{mcode}
%   type EmpyAShip = AShip <\_$\,$->$\,$False,\_$\,$->$\,$True>
%   type FullAShip = AShip <\_$\,$->$\,$True,\_$\,$->$\,$False>
%   type OrigAShip = AShip <\s$\,$->$\,$s = Ship$\,$0$\,$0,\s$\,$->$\,$s $\not =$ Ship$\,$0$\,$0>
% \end{mcode}
% %
% The positive predicate of @EmpyAShip@ states that all its elements should satisfy 
% @False@, thus it represents the empty abstract domain. 
% Dually, the negative predicate of @FullAShip@ states that all the elements 
% that do not belong to the domain should satisfy 
% @False@, thus it represents the full abstract domain. 
% %
% Finally, the predicates of @OrigAShip@ state that its elements 
% are exactly equal to @Ship 0 0@, which is satisfied only by the ship 
% that is positioned at the origin of the space.  
% The exact definition of abstract
% predicates~\citep{abstract-refinements} is provided
% in~\S~\ref{sec:encoding}, where it is also parameterized over any secret 
% data type. 
% Indexing the abstract domain with 
% these positive and negative predicates allows us to semantically reason 
% about the abstract domains decidably and without the need 
% to perform type level operations about \textit{each} element of the domain.

% The abstract domain must implement a set of operations 
% that, combined with the predicate indexes, let us specify 
% and prove that 
% the approximate \indsets
% under- or over-approximate the real 
% \indsets.
% For example, @AShip@ implements the three operations below. 
% \begin{mcode}
%   ($\in$) ::  Ship -> AShip -> Bool 
%   ($\subseteq$) :: AShip -> AShip -> Bool 
%   ($\cap$) :: AShip -> AShip -> AShip 
% \end{mcode}
% These operators are defined using the standard set-theoretic semantics, 
% \eg @Ship x y $\in$ AShip (Interval xl xh) (Interval yl yh)= xl <= x <= xh $\land$ yl <= y <= yh@.
% %\todo{come back here}
% % \jp{It'd be nice to use typeclasses here}

% Using the @AShip@ abstract domain, we can compute under- and over-approximations of the \indsets for the @nearby@ query as follows.
% \begin{mcode}
%   under_indset :: s: Ship ->
%    AShip<{\l -> nearby s <=> nearby l}, {\_ -> True}> 
%   under_indset s = case (nearby s)  of
%     True  -> AShip (Interval 121 279) (Interval 179 221) 
%     False -> AShip (Interval 0 400)   (Interval   0 99) 
% \end{mcode}
% % \jp{Do these numbers match the figure?}
% % \nv{nope!!!}
% @under_indset@ computes the under-approximation of
% the \indsets for @nearby@ as in Figure~\ref{fig:nearby:under}.
% The refinements on @under_indset@ state that for all secret @Ship@ inputs, 
% all elements in
% the returned abstract ship domain have the same result to @nearby@ as the secret input.
% At compile time, Liquid Haskell automatically proves that the returned abstract ship domain satisfies this refinement type.
% In other words, Liquid Haskell 
% % statically
% mechanically 
% proves that the returned abstract ship domain is an under-approximation of @nearby@'s \indset. % for the given secret input
% Dually, we define @over_indset@ which computes the over-approximation of @nearby@'s \indsets (\Cref{fig:nearby:over}). 
% \begin{mcode}
%   over_indset :: s:Ship -> 
%     AShip <{\_ -> True}, {\l -> $\lnot$(nearby s <=> nearby l)}>
%   over_indset s = case (nearby s) of
%     True  -> AShip (Interval 100 300) (Interval 100 300) 
%     False -> AShip (Interval 0 400)   (Interval 0 400)                                   
% \end{mcode}
% % \jp{Numbers correct?}\nv{no}
% The negative predicate in the type ensures
% that all the elements outside of the return abstraction 
% cannot match the @nearby@ query, thus it specifies super-sets 
% (\ie over-approximations) of the \indsets. 
% %
% Once again, Liquid Haskell automatically checks the specifications.

% % \jp{TODO: encode indistinguishability sets (move up soundIndSet and completeIndSet)}
% % \jp{TODO: encode under/over approximations w/ refinements, emphasize automatically, mechanically proven using LH}

% Ind. sets can directly used to prevent information leaks:
% when answering a query provided by the attacker, one can compute the \indsets and use them to determine whether disclosing the query result would violate the given security policy.
% % instead of providing the exact answer of a query to the attacker, 
% % one can compute and return the \indsets after validating that 
% % private information are not leaked. 
% Next, we use \indsets to compute track an attacker's knowledge. 

% \subsection{Modeling Knowledge Approximations}
% \label{subsec:knowledge}
% %
% % \jp{TODO: Background on knowledge + posteriors. Incorporate the comments (moved down from above)}
% % As a result, the larger an \indset is the more uncertain the attacker is about @nearby@'s input and, 
% % dually, a small \indset indicates that the attacker's uncertainty is low since there are only few possible elements in the set.
% %
% % Therefore, under-approximations provide a lower-bound on the
% % information learned by an attacker by observing the query result.
% %
% % That is,  over-approximations provide an
% % upper-bound on the attacker's uncertainty with respect to the input:
% % all inputs that do not belong to the over-approximated \indset do not belong to the original \indset.
% %
% % \jp{encode knowledge/belief (move up sound and complete)}
% %
% %
% %
% The \emph{knowledge} of an attacker (see \S~\ref{sec:security}) is the set of
% all possible secret values that are consistent with the attacker's
% observations~\cite{askarov2007gradual}. 
% For example, the attacker might already have some prior knowledge about the ship 
% location and might use the result of the @nearby@ query to refine this knowledge. 
% To compute the refined knowledge after the query, \aka the \textit{posterior} knowledge, 
% we simply intersect the prior knowledge with the \indset associated with the query result. 
% If the intersection happens with the real \indsets, then we derive 
% the real posterior. 
% Under-approximations of attacker knowledge provide a lower-bound on the
% information learned by an attacker by observing the query result.
% Dually, over-approximations of knowledge provide an upper-bound on the information learned by observing the query result.
% To computer the over- and under-approximations of posterior knowledge, 
% we intersect the prior knowledge respectively with the over- and under-approximations 
% of the \indsets.

% \paragraph{Knowledge under-approximation}
% An under-approximation of the posterior knowledge, with respect to @nearby@ and a
% secret value @s@, is an abstract 
% % knowledge 
% domain (@AShip@) whose elements agree with the
% response of @nearby s@ and belong to the prior knowledge @p@. The refinement type of a function that
% under-approximates this knowledge is:
% \begin{mcode}
%   under_post :: s:Ship -> p:AShip -> 
%     AShip <{\x -> (nearby s <=> nearby x) $\land$ (x $\in$ p)}
%           ,{\_ -> True}>
%   under_post s p = p $\cap$ under_indset s
% \end{mcode}
% The positive predicate specifies that all ships in the posterior 
% should have the same @nearby@ result as the secret and be elements of the prior knowledge.
% The negative predicate is @True@, since 
% we pose no requirements on the elements outside of the posterior. 
% % In~\S~\ref{sec:security}, we provide  definitions formalizing under- and over-approximations of knowledge that we use to derive the refinement-type encodings in~\S~\ref{sec:encoding}.

% \paragraph{Knowledge over-approximation}
% Dually, we generate an over-approximated posterior  
% as the intersection of prior with the over-approximated \indsets. 
% %
% \begin{mcode}
%   over_post  :: s:Ship -> p:AShip ->
%     AShip<{\_ -> True}
%          ,{\x -> (not (nearby s <=> nearby x)) $\lor$ (x $\not \in$ p)}>
%   over_post s p = p $\cap$ over_indset s
% \end{mcode}
% %   over_post secret prior = prior $\cap$ completeHelper secret prior
% %
% The specification of @over_post@ % encodes completeness since it 
% uses the negative index predicate to specify that 
% all the @Ships@ that do not belong in the result either differ from @s@ in their response to the @nearby@ query or do not belong to the prior @p@.
% %
% In~\S~\ref{sec:security}, we provide  definitions formalizing under- and over-approximations of knowledge that we use to derive the refinement-type encodings in~\S~\ref{sec:encoding}.


% % \begin{comment}
% \subsection{\tool: Approximate Knowledge Synthesis}
% \label{subsec:tool}
% %
% %\begin{wrapfigure}{r}{0.4\textwidth}
% %\begin{figure}
% %  \begin{center}
% %    \includegraphics[width=0.3\textwidth]{anosy}
% %  \end{center}
% %  \caption{\tool workflow.}
% %  \label{fig:tool:workflow}
% %\end{wrapfigure}
% %\end{figure}
% %
% % 
% % Our 
% % The refinement type 
% The
% encodings of \indsets (\S~\ref{subsec:indset}) and posterior knowledge (\S~\ref{subsec:knowledge}) verify the correctness of their over- and under-approximations. 
% Defining these approximations, however, is difficult, \eg it requires coming up with abstract domain elements (like in Figure~\ref{fig:nearby-example}) for each query. %but it is difficult to define 
% %them. 
% % these approximations. 
% % come up with their definitions. 
% %
% To aid in this task, we present \tool, an \underline{a}pproximate k\underline{no}wledge \underline{sy}nthesizer, which automatically synthesizes over- or under-approximations of
% \indsets and posterior knowledge
% for a given query. 
% % 
% % \tool is an \underline{a}pproximate k\underline{no}wledge \underline{sy}nthesizer whose workflow is 
% % presented in Figure~\ref{fig:tool:workflow}. 
% \Cref{fig:tool:workflow} shows the workflow of \tool. 
% \tool takes as input a query function @q@, 
% a secret @s@, and the attacker's prior knowledge @p@. 
% It uses the query and the secret to synthesize 
% the over- or under-approximations of the \indsets 
% and then intersects these with the prior knowledge 
% to  derive the attacker's % sound and complete 
% posterior knowledge. 
% Concretely, \tool is implemented as a GHC plugin that 
% takes as input annotated Haskell code 
% and returns a Haskell program  
% that includes definitions of the approximate \indsets and posterior knowledge. 
% % that is checked by Liquid Haskell to compute
% % knowledge approximations. 
% % \jp{LH verifies that the computed posterior distribution is sound/complete, right?}
% In the rest of this section, we present how 
% \tool works on the @nearby@ example. 
% %\begin{wrapfigure}{r}{0.4\textwidth}
% \begin{figure}
%   \begin{center}
%     \includegraphics[width=0.3\textwidth]{anosy}
%   \end{center}
%   \caption{\small \tool workflow.}
%   \label{fig:tool:workflow}
% %\end{wrapfigure}
% \end{figure}
% % \mg{Why do we need secret as input? Isn't it enough to get a query result? }
% % \jp{I agree. Can we remove the s input from fig 2? Maybe not since p is there too}

% \paragraph{\tool's input: Annotated Haskell Code}
% \tool takes as input Haskell code annotated to specify 
% what approximations will be generated and with respect to which 
% abstract domains. 
% For example, below we 
% % define the annotated @nearby@ query 
% re-present the definition of
% the @Ship@ data type and demonstrate its \tool annotation. 
% \begin{mcode}
%   data Ship = Ship { x :: Int, y :: Int}

%   {-# ANN Ship ([("x", (0, 400)), ("y", (0, 400))] 
%                  :: [(String, (Int, Int))]) #-}
% \end{mcode}
% The annotation states that 
% \tool should use the 
% interval % integer 
% range @(0,400)@ to abstract both the @x@ and @y@ fields of the @Ship@.

% Annotations are also used to declare what functions will be synthesized. 
% For example, the below annotation spacifies that \tool 
% should synthesize the over-approximation of the posterior 
% for the @nearby@ Haskell query. 
% \begin{mcode}
%   {-# ANN module ("over_post",  "nearby") #-}
% \end{mcode}
% % The @Ship@ data type contains two Integers that model
% % the ship's location. The first annotation states that each location 
% % will be abstracted by the integer range @(0,400)@ to generate the @Ship@
% % abstract domain. 
% % Then, the absolute value function is defined in the standard way 
% % and used to implement @nearby@ that decides if the input (secret) ship 
% % has Manhattan distance to @(200,200)@ less than or equal to @100@. 
% %The annotations specify that \tool 
% %should generate the over- and under-approximations of posterior knowledge
% %after running the @nearby@ query. 

% \paragraph{\tool's Output}
% The result of running \tool on the above input 
% will be a Haskell executable file that contains the @Ship@'s abstract domain definition (@AShip@), and
% over- and under-
% approximations of both the \indsets and posterior knowledges 
% as presented in~\S~\ref{subsec:indset} and \S~\ref{subsec:knowledge}. 
% That is, the output file contains both the correctness specifications 
% of the approximations and their implementations. 
% As a sanity check and to reduce the trusted codebase, 
% \tool runs Liquid Haskell on the output file to verify the generated code. 

% \paragraph{\tool's Synthesis}
% To generate the output Haskell file, \tool 
% combines metaprogramming, program sketching, and SMT-based synthesis. 
% First, using metaprogramming, it generates the type specifications of the functions 
% to be synthesized. 
% Next, using program sketching, it generates the function definitions templates 
% using synthesis variables for the difficult-to-generate 
% % literals
% integers 
% that define 
% the bounds of the 
% % interval abstractions. 
% abstract domains. 
% Finally, and based on the precise refinement-type specifications, 
% it generates integer constraints on the synthesis variables and uses 
% an SMT solver to solve these constraints, thus synthesizing the 
% % abstraction intervals. 
% abstract domains. 
% We elaborate on the synthesis process in~\S~\ref{sec:synthesis}. 


% \tool is able to automatically synthesize abstract domains for user defined 
% data types that contain integer fields. 
% In~\S~\ref{sec:evaluation}, we evaluate the precision of the synthesized 
% posteriors using intervals 
% and powerset of intervals as our abstract domains.
% % % , 
% % % while our 
% % \tool's implementation is extensible, making it generalizable to support
% % additional abstract domains. 
% % % with further abstraction domains. 

% \begin{comment}
% \paragraph{Abstract Domain Generation}
% The provided @Ship@ annotation is used to generate the 
% abstract domain of Ships in which each integer is 
% abstracted with an integer range. 
% %
% Concretely, the below two data type abstractions will be defined. 
% \begin{code}
%   data AbsInt = AbsInt { lower :: Int, upper :: Int}
%   data AbsShip <p :: Ship -> Bool, n :: Ship -> Bool> = AbsShip {
%     xr :: AbsInt
%   , yr :: AbsInt }
% \end{code}
% The @AbsInt@ simply defines the abstraction of an integer in
% the range between its @lower@ and @upper@ fields. 
% The @AbsShip@ defines an abstraction of the @Ship@ data type 
% where each field contains an integer abstraction. 

% Importantly, the @AbsShip@ data type is parameterized
% by two predicates to denote the elements it contains. The @p@ property is satisfied
% by all elements that belong to @AbsShip@, whereas @n@ describes all
% elements that lie outside @AbsShip@.
% For example, below we present the types that encode an empty, a full, and the origin 
% ship abstractions. 
% \begin{mcode}
%   type EmpyAbsShip = AbsShip <\_ -> False, \_ -> True>
%   type FullAbsShip = AbsShip <\_ -> True, \_ -> False>
%   type OrigAbsShip = AbsShip <\s -> s = Ship 0 0, \s -> s /= Ship 0 0>
% \end{mcode}
% %
% The positive predicate of @EmpyAbsShip@ states that all its elements should satisfy 
% @False@, thus it represents the empty abstract domain. 
% Dually, the negative predicate of @FullAbsShip@ states that all the elements 
% that do not belong to the domain should satisfy 
% @False@, thus it represents the full abstract domain. 
% %
% Finally, the predicates of @OrigAbsShip@ state that its elements 
% are exactly equal to @Ship 0 0@, which is satisfied only by the ship 
% that is positioned at the origin of the space.  
% The exact definition of abstract
% predicates~\citep{abstract-refinements} is provided
% in~\S~\ref{sec:encoding}. 
% Indexing the abstract domain with 
% these positive and negative predicates allows us to semantically reason 
% about the abstract domains decidably and without the need 
% to perform type level operations about \textit{each} element of the domain.

% Finally, the abstract domains come with a set of operations 
% that, combined with the predicate indexes, let us specify 
% and prove that the generated knowledge  under- or over-approximates the real knowledge. 
% \begin{mcode}
%   ($\in$) ::    C -> AbsC -> Bool 
%   ($\subseteq$) :: AbsC -> AbsC -> Bool 
%   ($\cap$) :: AbsC -> AbsC -> AbsC 
% \end{mcode}
% In the above @C@ can be either @Int@ or @Ship@ and 
% the operators are defined using the standard set-theoretic definitions, 
% \eg @i $\in$ AbsInt l h = l <= i <= h@.
% %\todo{come back here}





% \paragraph{Encoding of an under-approximation of the Posterior}
% An under-approximation of the  posterior, with respect to @nearby@ and a
% secret value @secret@, is an abstract knowledge (@AbsShip@) whose elements agree with the
% response of @nearby secret@. The refinement type of a function that
%  under-approximates the posterior is:
% \begin{mcode}
%   {-@ sound :: secret: Ship
%     -> {prior: AbsShip | secret $\in$ prior}
%     -> {post:  AbsShip<{p:Ship | nearby secret <=> nearby p},{\_ -> True}|post $\subseteq$ prior> 
%   @-}
% \end{mcode}
% The positive predicate of specifies that all ships in the result abstract domain 
% should have the same @nearby@ result as the secret. 
% The negative predicate is @True@, since 
% we pose no requirements on the  elements outside of the posterior. 
% Finally, the resulting posterior should be a subset of the prior knowledge.
% In~\S~\ref{sec:security} we provide a security-oriented definition 
% of under- and over-approximations of knowledge that we use to derive the refinement-type encodings in~\S~\ref{sec:encoding}.

% \mg{Update terminology in code snippets}

% \paragraph{Synthesising under-approximations}
% Defining under-approximations is tedious. For example, 
% below we present a user-provided definition of @sound@. 
% \begin{mcode}
%   sound secret (AbsShip (AbsInt xl xu) (AbsInt yl yu)) = 
%     case (nearby secret) of
%      True  -> AbsShip (AbsInt (max xl 188) (min xu 212))
%                       (AbsInt (max yl 112) (min yu 288))
%      False -> AbsShip (AbsInt (max xl 301) (min xu 500))
%                       (AbsInt (max yl   0) (min yu 500))
% \end{mcode}
% \todo{can we change this to be in the 400x400 plane and thus consistent with the figures}
% Writing this function is difficult and error prone for two reasons.
% First, we need to come up with the correct integers 
% (like @188@ and @212@ above), which normally 
% implies solving tedious arithmetic constraints. 
% Second, the code gets complicated because these integers are combined via 
% @min@ and @max@ with the coordinates of the prior argument. 

% The second problem has an easy solution: 
% instead of explicitly computing the posterior, we can express 
% it as an intersection of the prior with an under-approximation of the \indset. 
% Thus, the manual definition of the under-approximated posterior reduces to the following.
% %
% \begin{mcode}
%   sound :: Ship -> AbsShip -> AbsShip
%   sound secret prior = prior $\cap$ soundIndSet secret prior
% \end{mcode}
% %
% where @soundIndSet@ computes the under-approximation of 
% the \indsets with respect to @nearby@ (as in Figure~\ref{fig:nearby:under})
% \begin{mcode}
%   {-@ soundIndSet :: secret: Ship
%        -> {prior: AbsShip | secret $\in$ prior}
%        -> AbsShip<{l:Ship | nearby secret <=> nearby l}, {\_ -> True}> 
%   @-}
%   soundIndSet secret _ = case (nearby secret)  of
%     True  -> AbsShip (AbsInt 188 212) (AbsInt 112 288) 
%     False -> AbsShip (AbsInt 301 500) (AbsInt   0 500) 
% \end{mcode}
% %
% \mg{Prior is not needed as input in SoundIndSet, right?}
% % 
% The main challenge still remains: 
% coming up with the integers that specify the \indsets is a tedious procedure. 
% But, our use of the index predicates combined with the isolation of the
% prior dependencies, has set up a linear arithmetic synthesis problem 
% that is easily addressed by SMT solvers. 
% %
% In~\S~\ref{sec:synthesis} we explain how \tool uses SMT's synthesis and 
% optimization features to encode and synthesize correct \indsets. 
% Further, as explained in~\S~\ref{sec:implementation}, 
% \tool combines SMT-based synthesis with 
% metaprogramming to systematically generate
% correct-by-construction inhabitants of the @sound@ function.

% \paragraph{Encoding of an over-approximated Posterior}
% Dually, \tool will generate an over-approximated posterior  
% as the intersection of prior with the over-approximated \indsets. 
% %
% \begin{mcode}
%   {-@ complete :: secret: Ship
%   -> {prior: AbsShip | secret $\in$ prior}
%   -> AbsShip<{\_ -> True}, {l:Ship | $\lnot$ (nearby secret <=> nearby l) $\lor$ $\lnot$ (l $\in$ prior) }>
%   @-}
%   complete secret prior = prior $\cap$ completeHelper secret prior
% \end{mcode}
% %
% The specification of @complete@ encodes completeness since it 
% uses the negative index predicate to specify that 
% all the @Ships@ that do not belong in the result have different response 
% on the @nearby@ query that the respond of @secret@. 
% \nv{We do not need subset of prior?}\mg{In principle yes. Wouldn't that come for free from intersection?}
% \nv{sure... I meant: do we need the precondition that secret has to belong in the prior? It not there in section 4}

% \tool will use the SMT-based synthesis to generate the over-approximated \indset 
% depicted in Figure~\ref{fig:nearby:over} as follows 
% \begin{mcode}
%   {-@ completeIndSet :: secret: Ship
%        -> {prior: AbsShip | secret $\in$ prior}
%        -> {post:AbsShip<{\_ -> True}, {l:Ship | $\lnot$(nearby secret <=> nearby l) $\lor$ $\lnot$(l $\in$ prior) }> | true }
% @-}
% completeIndSet secret _ = case (nearby secret) of
%   True  -> AbsShip (AbsInt 100 300) (AbsInt 100 300) 
%   False -> AbsShip (AbsInt 0 400)   (AbsInt 0 400)                                   
% \end{mcode}



% \subsection{Summary}
% \tool comes uses metaprogramming and SMT-based integer synthesis 
% to derive correct-by-construction posteriors of user defined functions. 
% \todo{HERE based on the rest of the paper}

% \end{comment}


==> security.tex <==
\section{Background: Security model}
\label{sec:security}

%% TODO: 
%% Our goal is to use refinement types to encode
%% Here: Background on the accepted definitions.

In this section, we provide background on the standard 
mathematical formalization of indistinguishable sets and knowledge based on~\cite{askarov2012learning,backesleak09}.
%
We start by presenting general notation.
%
Next, we formalize \indsets and, afterwards, the knowledge of an attacker.
%
We conclude by providing a semantic characterization of  under- and over-approximations for both \indsets and knowledge.
In the next section, we encode these definitions using 
refinement types. 

\begin{figure}
    \begin{center}
      \includegraphics[width=0.3\textwidth]{knowledge_venn}
    \end{center}
    \vspace{-10pt}
    \caption{\small The knowledge ($K$) is the intersection of prior knowledge ($P$) with
             the \indset on $q$ for the secret $s$ ($q\ x = q\ s$).}
    \vspace{-15pt}
    \label{fig:posterior:knowledge}
\end{figure}

\paragraph{Setting}
%
We consider a set $\mathcal{S}$ containing all possible secret values.
%
For simplicity, we consider only programs $q :  \mathcal{S} \to
\texttt{Bool}$, which we call \emph{queries}, that take as input a secret
$s \in \mathcal{S}$ and outputs a boolean value.
%
All our definitions can be easily extended to handle additional
non-sensitive information and arbitrary output domains.
%
We consider an attacker that wants to infer information about a secret 
$s \in \mathcal{S}$ by observing the boolean results $o_1, \ldots, o_n$ of 
queries $q_1, \ldots, q_n$ that are all executed on $s$.


\paragraph{Indistinguishable sets}
%
A query $q$ partitions the set $\mathcal{S}$ into two \indsets 
$I_{q,\texttt{tt}}$ and $I_{q,\texttt{ff}}$ \resp 
for the true and false boolean results. 
%
Each \indset $I_{q,o}$ contains all secret values $s \in \mathcal{S}$ that produce the output $o$ in response to the query $q$.
%
That is, $I_{q,o} = \{ s\in \mathcal{S} \mid q\ s = o \}$.\footnote{$I_{q,\texttt{tt}}$ and $I_{q,\texttt{ff}}$ are the two equivalence classes induced by the indistinguishability equivalence relation $\sim_q$ such that $s \sim_q s'$ iff $q\ s = q\ s'$~\cite{backesleak09}.}
%
Hence, attackers (without further information) that observe the output $o$ only know that the secret is one of the values in $I_{q,o}$ but they cannot obtain further information.
%
% For simplicity, we write $I_{q}$ to denote the function that maps each output $o \in \mathcal{O}$ to the corresponding \indset $I_{q,o}$.

\paragraph{Attacker knowledge}
%
The knowledge of an attacker is the set of secrets that they consider
possible based on some initial prior knowledge and the results of multiple queries~\cite{askarov2007gradual}.
%
Initially, the knowledge is identical to the prior and it gets refined after each observation using the \indsets.

Let $s \in \mathcal{S}$ be the  secret and $\mathtt{P}
\subseteq \mathcal{S}$ be the \emph{prior knowledge}, i.e., the set of
all secrets the attacker consider possible before interacting with the
system. For simplicity, we assume that the secret $s$ belongs to the
prior. After observing that the result of a query $q$ is $o$, the
updated knowledge $\mathit{K}(o, \mathtt{P}, q)$, also called the
\emph{posterior knowledge}, is $\mathit{K}(o, \mathtt{P}, q) := \mathtt{P} \cap I_{q,o}$; see Figure~\ref{fig:posterior:knowledge} for a graphical depiction.
%
That is, $\mathit{K}(o, \mathtt{P}, q)$ is the set of all secrets that are consistent with both the prior and observing the output $o$ (captured by the \indset $I_{q,o}$).
The notion of knowledge can be generalized to sequences of $n$ queries $q_1
\cdot \ldots \cdot q_n$ with outputs $o_1 \cdot \ldots \cdot o_n$ as $
\mathit{K}(o_1 \cdot \ldots \cdot  o_n, \mathtt{P}, q_1 \cdot
\ldots \cdot q_n) := \mathit{K}(o_n, \mathit{K}(o_{n-1}, \ldots
\mathit{K}(o_2,  \mathit{K}(o_1, \mathtt{P}, q_1), q_2) \ldots)
q_{n-1}), q_n)
$ which is equivalent to $\mathit{K}(o_1 \cdot \ldots \cdot  o_n, \mathtt{P}, q_1 \cdot
\ldots \cdot q_n) := \mathtt{P} \cap I_{q_1,o_1} \cap \ldots \cap I_{q_n,o_n}$.

% \mg{Check terminology. Knowledge? Belief? Perhaps simply using prior and posterior}


\paragraph{Abstract domains}
%
Precisely representing \indsets and knowledge is, in general, an uncomputable task.
%
Hence, we approximate them using abstract domains  \adom over the set of secrets $\mathcal{S}$, which we introduce next.
%
We model an \emph{abstract domain} as a set \adom of abstract values equipped with three operations:
\begin{inparaenum}
\item a \emph{concretization function} $\gamma: \adom \to 2^{\mathcal{S}}$ that maps each abstract element to the set of concrete elements it represents,
\item an \emph{intersection function} $\sqcap: \adom \times \adom \to \adom$ that intersects two abstract elements, and
\item an \emph{ordering relation} $\sqsubseteq$ over $\adom \times \adom$ that orders abstract elements.
\end{inparaenum}
%
As standard, we require that $\absval \sqsubseteq \absval'$ iff $\gamma(\absval) \subseteq \gamma(\absval')$, $\absval \sqcap \absval' = \absval' \sqcap \absval$, 
and $\absval \sqcap \absval' \sqsubseteq \absval$.
%
We write $c \in \absval$, where $c$ is a concrete value in $\mathcal{S}$ and $\absval$ is an abstract value in $\adom$, when $c\in\gamma(\absval)$.




\paragraph{Approximating \indsets}
%
An \emph{approximation} for the \indsets induced by the query $q$ using the abstract domain $\adom$ is two abstract elements $\absval_{q,\texttt{tt}}$ and $\absval_{q,\texttt{ff}}$, 
\resp for the true and false query results. 
%
We say that $\absval_{q,\texttt{tt}}$ and $\absval_{q,\texttt{ff}}$ \emph{under-approximate} the \indsets $I_{q,\texttt{tt}}$ and $I_{q,\texttt{ff}}$
\textit{iff} $\gamma(\absval_{q,\texttt{tt}}) \subseteq I_{q,\texttt{tt}}$ and  $\gamma(\absval_{q,\texttt{ff}}) \subseteq I_{q,\texttt{ff}}$.
%
Dually, we say that $\absval_{q,\texttt{tt}}$ and $\absval_{q,\texttt{ff}}$ \emph{over-approximate} the \indsets $I_{q,\texttt{tt}}$ and $I_{q,\texttt{ff}}$ 
\textit{iff} $\gamma(\absval_{q,\texttt{tt}}) \supseteq I_{q,\texttt{tt}}$ and $\gamma(\absval_{q,\texttt{ff}}) \supseteq I_{q,\texttt{ff}}$.
%


\paragraph{Approximating knowledge}
%
Assume that the prior knowledge $\mathtt{P}$ is represented by an abstract element $\absval_{\mathtt{P}}$ and let $\absval_{q,\texttt{tt}}, \absval_{q,\texttt{ff}}$ 
be an approximation for the \indsets induced by the query $q$.
%
The  \emph{abstract posterior knowledge} after the attacker observed that $q$'s result is $o$ is simply $\absval_{\mathtt{P}} \sqcap \absval_{q, o}$.
%
Observe that if $\absval_{q,o}$ is an under-approximation, then the abstract posterior knowledge under-approximates the real one, 
\ie $\gamma(\absval_{\mathtt{P}} \sqcap \absval_{q, o}) \subseteq K(o, \gamma(a_{\mathtt{P}}), q)$.
%
Dually, if $\absval_{q,o}$ is an over-approximation, then the abstract posterior knowledge over-approximates the real one, \ie $\gamma(\absval_{\mathtt{P}} \sqcap \absval_{q, o}) \supseteq K(o, \gamma(a_{\mathtt{Prior}}), q)$.
%
So, using \indsets approximations, we can provide lower and upper bounds on the real knowledge.



% \mg{Fix notation with figure (\indset wrt output value or wrt secret)}

% \mg{I don't like that we're defining different operations and notation from overview}

% \mg{Using sequences of elements/sets is a bit of a mess. Would it be easier to understand if we say: query $q$ induces a function $I_q$ mapping each output $o$ to the \indset $I_{q,o}$ and approximation $appr$ is a function mapping each query $q$ and each output $o$ to $a_{q,o}$? Then, under/over approx is simply $\gamma(appr(q,o)) \subseteq I_q(o)$.}

% \subsection{Abstract Domains}

% Reasoning about knowledge requires one to reason about all secrets that
% belong to the knowledge set, an uncomputable task in general.
% Hence, we consider \emph{approximations} of knowledge represented via
% abstract domains \adom.

% \paragraph{Properties}

% Abstract domains model the (prior and posterior) knowledge as abstract
% elements $a \in \mathcal{A}$, each one mapped to a concrete set
% $\gamma(a)$ of secrets in $\mathcal{S}$. We define a partial order
% relation $\sqsubseteq$ for abstract domains such that $a_1 \sqsubseteq
% a_2$ iff $\gamma(a_1) \subseteq \gamma(a_2)$. \sng{there are other
% operations like $\in$, $\cap$ that we discuss in \S~\ref{sec:encoding},
% which if we introduce here might be repetative.}

% Therefore, an approximation of the posterior knowledge $\mathtt{apprx}$,
% takes as the observation $o \in \mathcal{O}$, an abstract prior $a  \in
% \mathcal{A}$,  and the query $q$, and output the abstract posterior $a
% \in \mathcal{A}$. We are now ready to formalize the under- and
% over-approximation.

% \begin{definition}[Under-approximation]
% An approximation $\mathtt{apprx} :  \mathcal{O} \times \mathcal{A}
% \times Prg \to \mathcal{A}$ is an \emph{under-approximation} if for all outputs $o \in
% \mathcal{O}$, priors $a \in \mathcal{A}$, and queries $p$, 
% $\gamma( \mathtt{apprx}(o,a,p) ) \subseteq \mathit{K}(o, \gamma(a), p)$.
% \end{definition}

% \begin{definition}[Over-approximation]
%     An approximation $\mathtt{apprx} :  \mathcal{S} \times \mathcal{A}
%     \times Prg \to \mathcal{A}$ is an \emph{over-approximation} if for all outputs
%     $o \in \mathcal{O}$, priors $a \in \mathcal{A}$, and queries $p$, 
%  $\mathit{K}(o, \gamma(a), p) \subseteq \gamma( \mathtt{apprx}(o, a, p) )$.
% \end{definition}

% \subsection{Applications}

% We now present various security-relevant applications of the knowledge
% and its approximations.

% \paragraph{Non-interference}

% Basic non-interference~\citep{goguennoninterference} requires that secret information
% \emph{does not} influence the computation's observable result.
% In our setting, non-interference is equivalent to requiring that
% $\mathit{K}(o, \mathcal{S}, p) = \mathcal{S}$  for all outputs $o \in
% \mathcal{O}$. That is, the attacker does not learn \emph{anything} about
% the secret by observing query $p$'s output.

% To \emph{soundly} check non-interference, one can use a sound
% approximation $\mathtt{approx}$ as follows: $\mathtt{approx}(o, \top, p)
% = \top$  for all outputs $o \in \mathcal{O}$, where $\top \in
% \mathcal{A}$ is the top element in the abstract domain. 


% \paragraph{Knowledge-based policies}
% %
% Knowledge-based policies \sng{cite?} express a bound on what information an
% attacker can infer from observing the computation's result. 
% In our setting, a knowledge-based policy can be represented as a set of
% secrets $\mathtt{Pol} \subseteq \mathcal{S}$ that should always be
% indistinguishable for the attacker.
% A query $p$  complies with a policy $\mathtt{Pol}$ iff for all priors
% $\mathtt{Prior}$, if $\mathtt{Pol} \subseteq \mathtt{Prior}$, then
% $\mathtt{Pol} \subseteq \mathit{K}(o, \mathtt{Prior}, p)$  for all
% outputs $o \in \mathcal{O}$. 

% Similar to non-interference, we can use a sound approximation to check
% for policy compliance. Specifically, we just need to find an abstract
% element $a \in \adom$ such that $\gamma(a) \subseteq \mathtt{Pol}$
% and check if $a \sqsubseteq \mathtt{approx}(o, \mathtt{Prior}, p)$  for
% all outputs $o \in \mathcal{O}$.

% % \mg{It might make sense to have a paragraph on abstract domains, notation, and properties like $a \sqsubseteq b \rightarrow \gamma(a) \subseteq \gamma(b)$.}

% \paragraph{Quantitative Information Flow}

% Quantitative information-flow~\sng{cite?} aims at quantifying the amount of
% information leaked by a computation. While several measures have been
% proposed for QIF, like Bayes vulnerability~\citep{smith2009foundations},
% Guessing entropy~\citep{massey1994guessing}, and Shannon
% entropy~\citep{shannon2001mathematical}, here we consider a criterion
% based on Shannon's entropy. Given two random variables $S$ representing
% the secrets and $O$ representing the computation output, the information
% leaked $L$ by the program $p$ is the mutual information between $S$ and
% $O$:
% \begin{align*}
%     H(S) &:= - \sum_{s \in S} Pr[O = o] \mathit{log}_2 Pr[S = s]\\
%     H(S \mid O) &:= \sum_{o \in O} Pr[O = o]  H(S \mid O = o)\\
%     L &:= H(S) - H(S \mid O)
% \end{align*}
% %
% \sng{is the 2nd eqn above correct?} The maximal leak is obtained when
% secrets are uniformly distributed. In this case, we can rewrite $L$ as
% follows:
% \begin{align*}
%     H(S) &:=  \mathit{log}_2 (|\mathcal{S}|)\\
%     H(S \mid O) &:= \sum_{o \in O} |\{ s \in \mathcal{S} \mid  p(s) = o\}|^{-1}  \mathit{log}_2(|\{ s \in \mathcal{S} \mid  p(s) = o\}|)\\
%     L &:= H(S) - H(S \mid O)
% \end{align*}
% %
% Observe that $\{ s \in \mathcal{S} \mid  p(s) = o\}$ is, effectively,
% $\mathit{K}(o, \mathcal{S}, p)$, which we can approximate using a sound
% approximation $\mathtt{approx}$. \sng{This seems disconnected with the
% paper, but i am not sure how to fix}




% \mg{Could we also have a timing-based QIF adversary here? We just need
% to output the number of ``evaluation ticks''!} \sng{cite niki's
% performance verification with liquid types paper?}

% \mg{I need to check again the math and the directions of the approximation!}

% % \paragraph{Secret protection}
% % %
% % Secrecy policies~\cite{} specify predicates $\phi$ to be kept secret, that is, an attacker should not be able to infer $\phi$'s truth value.
% % %
% % In our setting, we represent the predicate $\phi$ as the set of secrets that satisfy it.
% % %
% % A query $p$ preserves the secret $\phi$ if for all secrets $s$, there is a secret $s'$ such that $p(s) = p(s')$ and $|\{ s, s' \} \cap \phi| = 1$.
% % %
% % \mg{Is there a connection with secrets?}


% \mg{We need an application for completeness :-/ Difficult!}
% \mg{The only use case that I have, so far, for completeness is making sure that an attacker doesn't consider some value as possible. For this, we would need to consider the over-approximation rather than the under-approximation. Still, it's a rather sketchy idea which I'm not sure has ever been studied in the literature.}

% \mg{The perfect use case for over-approximation is comparing leakages! We want to check if one query leaks more than another. For this we need to compare the over-approx of the first and the under-approx of the second!}

% \jp{Could compute QIF metrics like entropy using synthesized posteriors.}


==> synthesis.old.tex <==
\section{Synthesis of Secure Domains}
\label{sec:synthesis}

As seen from the previous examples, coming up with over-approximate or
under-approximate posteriors can often be a tedious and time-consuming
task, prone to mistakes. While the type system design in
\S~\ref{sec:encoding} allows us to verify is our posteriors are correct
for a query, we can go a step further by synthesizing secure posteriors.

Using a complete program synthesis method in our domain turns out to be
challenging because generating terms for each individual field of the
abstract domain would require reasoning about functions. Instead \tool
uses a method inspired by \emph{sketching} \sng{cite?}, where-in it
starts off with a partial program, that gives enough structure to the
problem. The remainder holes can be filled in by solving a much simpler
synthesis problem.

\subsection{Synthesis Sketch}

Given the refinement type of soundness and completeness, the following
sketch turns out be general enough to capture all kinds of solutions:
\mg{Do we have some intuition to back-up the generality claim?}
\begin{mcode}
  sound secret prior = prior $\cap$ _
\end{mcode}

Here the @_@ acts as a hole, that can be filled with terms that
eventually will satisfy the refinement type of sound. To simplify the
problem further, we rewrite the hole into a helper function application:

\begin{mcode}
  sound secret prior = prior $\cap$ (soundHelper secret)

  -- TODO: insert type of soundHelper here
  soundHelper secret = case ($\query$ secret) of
    True  -> _trueCase
    False -> _falseCase
\end{mcode}

In this rewritten form the hole @_trueCase@ corresponds
to an instance from our abstract domain that is under-approximation
of the region in which the query is true. Similarly, @_falseCase@ is the
under-approximation for the region which corresponds to the query
resulting in false case. As a result, this is considerably simpler
synthesis problem as these domains depend on just the query \query and
not the prior. Moreover, since they just depend on the query only, these
abstract domains can be constructed from integer constants, without
actually constructing terms from the prior. A similar decomposition can
be done for the complete posteriors as well.

\subsection{Synthesizing Constants}

Running type inference on the @_trueCase@ hole yields us
(\ref{eq:syn-sound-true}), which in other words says for all points
inside the @_trueCase@ will only evaluate to @True@ under the query
\query. We do not care if some points that can evaluate to @True@ are
not in this domain, \ie this domain is an under-approximation.
Similarly, (\ref{eq:syn-sound-false}) will hold for a domain in
which all points evaluate to @False@ under the query \query.

\begin{align}
\begin{split}
\forall \concval: \cdom. (\concval \in \texttt{\_trueCase}) \implies \query\ \concval \label{eq:syn-sound-true}
\end{split}
\\
\begin{split}
\forall \concval: \cdom. (\concval \in \texttt{\_falseCase}) \implies \lnot(\query\ \concval) \label{eq:syn-sound-false}
\end{split}
\\
\begin{split}
\forall \concval: \cdom. \query\ \concval \implies (\concval \in \texttt{\_trueCase}) \label{eq:syn-complete-true}
\end{split}
\\
\begin{split}
\forall \concval: \cdom. \lnot(\query\ \concval) \implies (\concval \in \texttt{\_falseCase}) \label{eq:syn-complete-false}
\end{split}
\end{align}

Completeness for the @_trueCase@ given by (\ref{eq:syn-complete-true})
says that all points which evaluate to @True@ under the query \query
should be in the @_trueCase@ domain. In other words, we do not care if
this domain contains some points that evaluate to @False@ as long as it
contains all the points that evaluate to @True@, \ie this is an
over-approximation. Similarly, (\ref{eq:syn-complete-false}) gives the
condition for the domain of completeness evaluating to @False@.


\paragraph{Optimization}

Running the above queries in a SMT solver will yield us some values for
the bounds of the abstract domain in the form of integer constants.
\sng{give an example or refer to \S~\ref{sec:overview}}. But often the
values will be correct but not necessarily a good choice, as we would
want our domains to be as big as possible so that it represents the most
amount of knowledge.

We use optimization support from Z3 to maximize our domains. Z3
optimization support works well for linear objectives, so we provide
the optimization goal as maximizing the ranges along all the dimensions of the
abstract domain. So for example if our abstract domain has @n@
dimensions, the optimization directive is:

\begin{mcode}
  (maximize (- $x_1^{max}$ $x_1^{min}$))
  $\dots$
  (maximize (- $x_n^{max}$ $x_n^{min}$))
\end{mcode}

This gives us a domain that is maximized on all dimensions along the
pareto front together \sng{not just one dimension maximized followed by
another and so on}

\mg{This part would benefit from some more details: what are max and mix values? what is the underlying domain? How do we maximize other domains?}

\subsection{Lifting back to Haskell}

Once we have the synthesized model from Z3, we translate the terms back
to Haskell by constructing the terms using these integer constants:

\begin{mcode}
  _trueCase  = Range [(IntRange 188 212), (IntRange 112 288)] propTruePos  propEmpty
  _falseCase = Range [(IntRange 301 500), (IntRange   0 500)] propFalsePos propEmpty
\end{mcode}

Here @propTruePos@, @propFalsePos@, @propEmpty@ are proof terms required
for the automatic verification to go through. These terms are
boilerplate, just checking that each field of the secret are inside the
bounds or not. Hence, these are produced by \tool automatically:

\begin{mcode}
  {-@ propTruePos :: li:{Secret | 188 <= x li && x li <= 212 && 112 <= y li && y li <= 288}
                  -> {l:Secret <{v:Secret | True <=> query v}> | l = li} @-}
  propTruePos :: Secret -> Secret 
  propTruePos li = li

  {-@ propFalsePos :: li:{Secret | 301 <= x li && x li <= 500 && 0 <= y li && y li <= 500}
                   -> {l:Secret<{v:Secret | False <=> query v}> | l = li }  @-}
  propFalsePos :: Secret -> Secret 
  propFalsePos li = li

  {-@ propEmpty :: li:Secret -> {lr:Secret | li = lr } @-}
  propEmpty :: Secret -> Secret 
  propEmpty li = li
\end{mcode}

